The Orbital Eccentricity--Radius Distribution for Warm, Single Planets in TESS

We characterize the radius-dependent eccentricity distribution of 219 warm (P = 8--50 days) systems with only one transiting planetary candidate identified during Sectors 1-69 of the TESS mission. Using the ``photoeccentric effect'' in a hierarchical Bayesian framework, we first model the population using discrete planetary size bins (sub-Neptunes, sub-Saturns, and Jovians). We then develop a continuous mixture model with weights governed by a logistic sigmoid function of radius. We find that the warm-single population is best described by two components: a dominant low-eccentricity mode ( <e_low> = 0.039-0.038+0.018) and a secondary dynamically excited mode (<e_high> = 0.466-0.068+0.067). The fraction of planets belonging to this high-eccentricity component increases strongly with planet radius, characterized by a transition at a break radius of R_br = 9.2-1.1+1.9 R_e. This trend places warm sub-Saturns predominantly on the same low-eccentricity track as sub-Neptunes. In contrast, warm Jovians (8--16 R_e) are frequently eccentric, with 65-12+13% of the population in the high eccentricity mode. Under the assumption of a two-component model, we see tentative evidence for a bimodal Jovian distribution at ~2.7 sigma. Finally, we identify a non-negligible tail of highly eccentric sub-Neptunes (1--4 R_e), which comprise 16.2-6.4+5.2% of the population, consistent with excitation by non-transiting external companions.

==> SINGLE_TABLE_MODE.tex <==
4897275 & 1774.01 &  & $1.143_{-0.031}^{+0.031}$ & $0.635_{-0.090}^{+0.090}$ & $0.39_{-0.28}^{+0.25}$ & $0.0234_{-0.0018}^{+0.0025}$ & $2.96_{-0.28}^{+0.28}$ & $0.49_{-0.34}^{+0.34}$ & $16.685_{-0.011}^{+0.011}$ & $1872.3338_{-0.0066}^{+0.0066}$ & $0.00_{-0.00}^{+0.39}$ & $-40_{-130}^{+30}$ \\
7422496 & 4189.01 &  & $0.891_{-0.020}^{+0.020}$ & $1.25_{-0.12}^{+0.12}$ & $1.09_{-0.57}^{+0.37}$ & $0.02607_{-0.00088}^{+0.00094}$ & $2.54_{-0.10}^{+0.11}$ & $0.45_{-0.30}^{+0.27}$ & $46.96229_{-0.00022}^{+0.00022}$ & $1470.3634_{-0.0026}^{+0.0026}$ & $0.03_{-0.03}^{+0.28}$ & $-30_{-150}^{+30}$ \\
9348006 & 1775.01 & TOI-1775 b & $0.834_{-0.021}^{+0.021}$ & $1.55_{-0.16}^{+0.16}$ & $1.28_{-0.40}^{+0.27}$ & $0.0900_{-0.0027}^{+0.0028}$ & $8.20_{-0.32}^{+0.31}$ & $0.37_{-0.24}^{+0.21}$ & $10.240544_{-0.000053}^{+0.000053}$ & $2635.3643_{-0.0011}^{+0.0011}$ & $0.01_{-0.01}^{+0.27}$ & $-20_{-140}^{+10}$ \\
14336130 & 1716.01 & TOI-1716.01 & $1.228_{-0.027}^{+0.027}$ & $0.543_{-0.082}^{+0.082}$ & $0.64_{-0.49}^{+0.38}$ & $0.0218_{-0.0016}^{+0.0032}$ & $3.06_{-0.39}^{+0.27}$ & $0.53_{-0.36}^{+0.33}$ & $8.082323_{-0.000053}^{+0.000053}$ & $2959.2194_{-0.0063}^{+0.0063}$ & $0.03_{-0.03}^{+0.35}$ & $-150_{-110}^{+330}$ \\
21832928 & 2128.01 & TOI-2128 b & $1.130_{-0.024}^{+0.024}$ & $0.770_{-0.087}^{+0.087}$ & $0.68_{-0.51}^{+0.36}$ & $0.0162_{-0.0009}^{+0.0014}$ & $2.03_{-0.17}^{+0.13}$ & $0.51_{-0.34}^{+0.33}$ & $16.34126_{-0.00013}^{+0.00013}$ & $1987.2721_{-0.0047}^{+0.0047}$ & $0.03_{-0.03}^{+0.32}$ & $-30_{-140}^{+50}$ \\
23229805 & 4451.01 &  & $1.137_{-0.022}^{+0.022}$ & $0.669_{-0.095}^{+0.095}$ & $0.56_{-0.22}^{+0.16}$ & $0.0330_{-0.0023}^{+0.0024}$ & $4.10_{-0.34}^{+0.26}$ & $0.42_{-0.28}^{+0.22}$ & $8.851711_{-0.000029}^{+0.000029}$ & $2778.5504_{-0.0011}^{+0.0011}$ & $0.00_{-0.00}^{+0.30}$ & $-150_{-20}^{+150}$ \\
23434737 & 1203.01 &  & $1.146_{-0.035}^{+0.035}$ & $0.65_{-0.11}^{+0.11}$ & $0.46_{-0.28}^{+0.25}$ & $0.0250_{-0.0012}^{+0.0013}$ & $3.14_{-0.19}^{+0.17}$ & $0.53_{-0.34}^{+0.25}$ & $25.502693_{-0.000085}^{+0.000085}$ & $1553.0764_{-0.0043}^{+0.0043}$ & $0.05_{-0.05}^{+0.31}$ & $-140_{-30}^{+130}$ \\
24358417 & 2338.01 & TOI-2338 b & $1.098_{-0.026}^{+0.026}$ & $0.699_{-0.093}^{+0.093}$ & $2.25_{-0.48}^{+0.82}$ & $0.1006_{-0.0018}^{+0.0014}$ & $12.00_{-0.33}^{+0.35}$ & $0.60_{-0.14}^{+0.07}$ & $22.653905_{-0.000049}^{+0.000049}$ & $2183.6804_{-0.0011}^{+0.0011}$ & $0.42_{-0.15}^{+0.21}$ & $130_{-110}^{+30}$ \\
25799609 & 963.01 &  & $1.078_{-0.026}^{+0.026}$ & $0.82_{-0.10}^{+0.10}$ & $0.57_{-0.39}^{+0.39}$ & $0.0563_{-0.0043}^{+0.0068}$ & $6.82_{-0.73}^{+0.59}$ & $0.54_{-0.36}^{+0.29}$ & $11.11783_{-0.00012}^{+0.00012}$ & $2235.0980_{-0.0070}^{+0.0070}$ & $0.01_{-0.01}^{+0.37}$ & $-30_{-140}^{+30}$ \\
29857954 & 172.01 & TOI-172 b & $1.812_{-0.060}^{+0.060}$ & $0.221_{-0.026}^{+0.026}$ & $0.51_{-0.15}^{+0.10}$ & $0.0585_{-0.0014}^{+0.0013}$ & $11.55_{-0.48}^{+0.44}$ & $0.36_{-0.24}^{+0.20}$ & $9.476879_{-0.000016}^{+0.000016}$ & $1326.9217_{-0.0015}^{+0.0015}$ & $0.30_{-0.11}^{+0.24}$ & $30_{-20}^{+130}$ \\
30037565 & 1209.01 &  & $1.344_{-0.027}^{+0.027}$ & $0.452_{-0.057}^{+0.057}$ & $2.2_{-1.6}^{+1.0}$ & $0.0177_{-0.0009}^{+0.0013}$ & $2.63_{-0.18}^{+0.17}$ & $0.48_{-0.33}^{+0.35}$ & $40.71961_{-0.00019}^{+0.00019}$ & $1337.0967_{-0.0053}^{+0.0053}$ & $0.55_{-0.17}^{+0.20}$ & $70_{-48}^{+88}$ \\
33831980 & 806.01 &  & $0.596_{-0.019}^{+0.019}$ & $2.87_{-0.30}^{+0.30}$ & $2.2_{-1.4}^{+1.1}$ & $0.0372_{-0.0019}^{+0.0029}$ & $2.46_{-0.18}^{+0.17}$ & $0.49_{-0.33}^{+0.29}$ & $21.916713_{-0.000091}^{+0.000091}$ & $1346.0110_{-0.0047}^{+0.0047}$ & $0.00_{-0.00}^{+0.35}$ & $-30_{-150}^{+20}$ \\
37770169 & 470.01 & TOI-470 b & $0.832_{-0.021}^{+0.021}$ & $1.44_{-0.16}^{+0.16}$ & $1.84_{-0.95}^{+0.71}$ & $0.0472_{-0.0020}^{+0.0023}$ & $4.30_{-0.21}^{+0.22}$ & $0.46_{-0.31}^{+0.26}$ & $12.191489_{-0.000048}^{+0.000048}$ & $1474.4938_{-0.0021}^{+0.0021}$ & $0.05_{-0.05}^{+0.29}$ & $-10_{-20}^{+190}$ \\
38571020 & 721.01 &  & $1.247_{-0.026}^{+0.026}$ & $0.588_{-0.090}^{+0.090}$ & $0.53_{-0.41}^{+0.35}$ & $0.0169_{-0.0012}^{+0.0020}$ & $2.37_{-0.25}^{+0.21}$ & $0.53_{-0.36}^{+0.34}$ & $12.287755_{-0.000087}^{+0.000087}$ & $3144.5636_{-0.0095}^{+0.0095}$ & $0.05_{-0.05}^{+0.33}$ & $-160_{-20}^{+170}$ \\
46104747 & 6535.01 &  & $1.877_{-0.055}^{+0.055}$ & $0.178_{-0.034}^{+0.034}$ & $1.06_{-0.96}^{+0.87}$ & $0.048_{-0.005}^{+0.025}$ & $12.6_{-3.6}^{+2.4}$ & $0.59_{-0.40}^{+0.37}$ & $20.83604_{-0.00015}^{+0.00015}$ & $3020.2150_{-0.0065}^{+0.0065}$ & $0.65_{-0.25}^{+0.19}$ & $70_{-50}^{+89}$ \\
48031665 & 4588.01 &  & $1.614_{-0.041}^{+0.041}$ & $0.400_{-0.045}^{+0.045}$ & $0.71_{-0.41}^{+0.27}$ & $0.01889_{-0.00091}^{+0.00096}$ & $3.33_{-0.19}^{+0.18}$ & $0.45_{-0.31}^{+0.29}$ & $13.11892_{-0.00010}^{+0.00010}$ & $1689.1341_{-0.0063}^{+0.0063}$ & $0.23_{-0.23}^{+0.20}$ & $0_{-10}^{+170}$ \\
49254857 & 4914.01 & TOI-4914 b & $1.015_{-0.028}^{+0.028}$ & $0.97_{-0.11}^{+0.11}$ & $5.0_{-0.9}^{+2.3}$ & $0.1124_{-0.0048}^{+0.0031}$ & $12.31_{-0.58}^{+0.52}$ & $0.77_{-0.11}^{+0.04}$ & $10.600573_{-0.000018}^{+0.000018}$ & $2317.2723_{-0.0011}^{+0.0011}$ & $0.62_{-0.20}^{+0.16}$ & $85_{-58}^{+75}$ \\
49428710 & 5174.01 & TOI-5174 b & $1.119_{-0.031}^{+0.031}$ & $0.69_{-0.10}^{+0.10}$ & $0.56_{-0.30}^{+0.19}$ & $0.0395_{-0.0018}^{+0.0023}$ & $4.86_{-0.31}^{+0.26}$ & $0.43_{-0.30}^{+0.29}$ & $12.21943_{-0.00038}^{+0.00038}$ & $2527.2972_{-0.0025}^{+0.0025}$ & $0.00_{-0.00}^{+0.32}$ & $-150_{-20}^{+150}$ \\
53189332 & 660.01 & WASP-106 b & $1.465_{-0.040}^{+0.040}$ & $0.377_{-0.039}^{+0.039}$ & $0.391_{-0.083}^{+0.061}$ & $0.0758_{-0.0009}^{+0.0010}$ & $12.13_{-0.37}^{+0.36}$ & $0.34_{-0.21}^{+0.16}$ & $9.289702_{-0.000010}^{+0.000010}$ & $1544.65099_{-0.00081}^{+0.00081}$ & $0.01_{-0.01}^{+0.23}$ & $-10_{-170}^{+40}$ \\
55559618 & 695.01 &  & $0.819_{-0.021}^{+0.021}$ & $1.62_{-0.17}^{+0.17}$ & $1.02_{-0.66}^{+0.51}$ & $0.0273_{-0.0011}^{+0.0015}$ & $2.46_{-0.13}^{+0.14}$ & $0.52_{-0.35}^{+0.28}$ & $21.376343_{-0.000054}^{+0.000054}$ & $1346.4093_{-0.0024}^{+0.0024}$ & $0.04_{-0.04}^{+0.34}$ & $-40_{-120}^{+20}$ \\
58723861 & 5120.01 &  & $1.466_{-0.037}^{+0.037}$ & $0.327_{-0.055}^{+0.055}$ & $0.540_{-0.078}^{+0.035}$ & $0.0735_{-0.0011}^{+0.0011}$ & $11.76_{-0.32}^{+0.36}$ & $0.19_{-0.13}^{+0.18}$ & $24.91631_{-0.00023}^{+0.00023}$ & $3267.9263_{-0.0067}^{+0.0067}$ & $0.23_{-0.14}^{+0.21}$ & $170_{-160}^{+0}$ \\
62483237 & 139.01 & TOI-139 b & $0.676_{-0.016}^{+0.016}$ & $2.28_{-0.20}^{+0.20}$ & $4.8_{-3.0}^{+2.3}$ & $0.0327_{-0.0024}^{+0.0032}$ & $2.45_{-0.23}^{+0.19}$ & $0.45_{-0.31}^{+0.33}$ & $11.084379_{-0.000098}^{+0.000098}$ & $1334.5470_{-0.0095}^{+0.0095}$ & $0.31_{-0.27}^{+0.19}$ & $20_{-20}^{+150}$ \\
66561343 & 892.01 & TOI-892 b & $1.435_{-0.035}^{+0.035}$ & $0.378_{-0.051}^{+0.051}$ & $0.422_{-0.081}^{+0.042}$ & $0.0786_{-0.0014}^{+0.0015}$ & $12.32_{-0.37}^{+0.38}$ & $0.24_{-0.17}^{+0.20}$ & $10.626600_{-0.000032}^{+0.000032}$ & $2219.5526_{-0.0014}^{+0.0014}$ & $0.03_{-0.03}^{+0.23}$ & $-10_{-20}^{+190}$ \\
67630845 & 2408.01 &  & $0.758_{-0.019}^{+0.019}$ & $1.84_{-0.18}^{+0.18}$ & $1.28_{-0.71}^{+0.74}$ & $0.0666_{-0.0051}^{+0.0070}$ & $5.62_{-0.56}^{+0.46}$ & $0.56_{-0.37}^{+0.23}$ & $9.463636_{-0.000040}^{+0.000040}$ & $2128.2975_{-0.0020}^{+0.0020}$ & $0.01_{-0.01}^{+0.36}$ & $-150_{-20}^{+140}$ \\
67711670 & 6033.01 &  & $1.464_{-0.036}^{+0.036}$ & $0.365_{-0.045}^{+0.045}$ & $0.44_{-0.18}^{+0.13}$ & $0.0711_{-0.0023}^{+0.0028}$ & $11.41_{-0.54}^{+0.44}$ & $0.42_{-0.28}^{+0.23}$ & $18.0422_{-0.0034}^{+0.0034}$ & $2885.9797_{-0.0027}^{+0.0027}$ & $0.05_{-0.05}^{+0.25}$ & $-160_{-130}^{+340}$ \\
68577662 & 4606.01 & K2-232 b & $1.209_{-0.029}^{+0.029}$ & $0.69_{-0.12}^{+0.12}$ & $0.675_{-0.029}^{+0.015}$ & $0.08788_{-0.00046}^{+0.00048}$ & $11.60_{-0.27}^{+0.28}$ & $0.11_{-0.08}^{+0.10}$ & $11.168409_{-0.000068}^{+0.000068}$ & $2522.95388_{-0.00025}^{+0.00025}$ & $0.00_{-0.00}^{+0.22}$ & $-20_{-160}^{+20}$ \\
71431780 & 1723.01 & TOI-1723 b & $1.098_{-0.019}^{+0.019}$ & $0.73_{-0.10}^{+0.10}$ & $0.90_{-0.53}^{+0.31}$ & $0.0272_{-0.0015}^{+0.0021}$ & $3.31_{-0.25}^{+0.19}$ & $0.43_{-0.29}^{+0.32}$ & $13.72703_{-0.00014}^{+0.00014}$ & $3307.767_{-0.014}^{+0.014}$ & $0.03_{-0.03}^{+0.30}$ & $-170_{-130}^{+350}$ \\
73038411 & 978.01 &  & $1.548_{-0.034}^{+0.034}$ & $0.321_{-0.056}^{+0.056}$ & $0.82_{-0.12}^{+0.05}$ & $0.0712_{-0.0010}^{+0.0010}$ & $12.03_{-0.33}^{+0.29}$ & $0.19_{-0.13}^{+0.17}$ & $13.166014_{-0.000021}^{+0.000021}$ & $2977.37828_{-0.00086}^{+0.00086}$ & $0.36_{-0.12}^{+0.22}$ & $150_{-140}^{+10}$ \\
76228620 & 4998.01 &  & $1.366_{-0.031}^{+0.031}$ & $0.395_{-0.061}^{+0.061}$ & $0.31_{-0.14}^{+0.28}$ & $0.0690_{-0.0068}^{+0.0057}$ & $10.17_{-0.98}^{+0.96}$ & $0.66_{-0.38}^{+0.14}$ & $9.7803490_{-0.0000060}^{+0.0000060}$ & $2378.92360_{-0.00065}^{+0.00065}$ & $0.01_{-0.01}^{+0.36}$ & $-30_{-150}^{+30}$ \\
80682484 & 2810.01 &  & $1.042_{-0.023}^{+0.023}$ & $0.84_{-0.11}^{+0.11}$ & $0.47_{-0.32}^{+0.21}$ & $0.0218_{-0.0010}^{+0.0019}$ & $2.54_{-0.18}^{+0.17}$ & $0.50_{-0.34}^{+0.32}$ & $8.403561_{-0.000048}^{+0.000048}$ & $3024.2893_{-0.0021}^{+0.0021}$ & $0.13_{-0.13}^{+0.29}$ & $-40_{-120}^{+10}$ \\
82308728 & 1821.01 & HD 97658 b & $0.756_{-0.028}^{+0.028}$ & $1.87_{-0.26}^{+0.26}$ & $1.8_{-1.1}^{+0.7}$ & $0.0282_{-0.0010}^{+0.0023}$ & $2.40_{-0.17}^{+0.16}$ & $0.48_{-0.32}^{+0.31}$ & $9.489330_{-0.000032}^{+0.000032}$ & $2664.08570_{-0.00085}^{+0.00085}$ & $0.00_{-0.00}^{+0.33}$ & $-160_{-20}^{+170}$ \\
85242435 & 1722.01 &  & $1.113_{-0.023}^{+0.023}$ & $0.83_{-0.10}^{+0.10}$ & $0.79_{-0.35}^{+0.18}$ & $0.0374_{-0.0011}^{+0.0013}$ & $4.56_{-0.19}^{+0.16}$ & $0.38_{-0.26}^{+0.27}$ & $9.605265_{-0.000020}^{+0.000020}$ & $3323.3233_{-0.0018}^{+0.0018}$ & $0.00_{-0.00}^{+0.28}$ & $-150_{-30}^{+160}$ \\
86273567 & 3858.01 &  & $1.167_{-0.026}^{+0.026}$ & $0.729_{-0.081}^{+0.081}$ & $0.68_{-0.45}^{+0.34}$ & $0.0424_{-0.0034}^{+0.0046}$ & $5.50_{-0.54}^{+0.53}$ & $0.49_{-0.32}^{+0.32}$ & $16.59684_{-0.00037}^{+0.00037}$ & $2606.4868_{-0.0050}^{+0.0050}$ & $0.02_{-0.02}^{+0.33}$ & $-30_{-150}^{+40}$ \\
87216634 & 5789.01 &  & $0.822_{-0.028}^{+0.028}$ & $1.61_{-0.19}^{+0.19}$ & $10.3_{-7.0}^{+5.5}$ & $0.0275_{-0.0018}^{+0.0023}$ & $2.50_{-0.20}^{+0.19}$ & $0.48_{-0.33}^{+0.33}$ & $12.9278_{-0.0038}^{+0.0038}$ & $2776.2544_{-0.0027}^{+0.0027}$ & $0.65_{-0.20}^{+0.14}$ & $106_{-85}^{+42}$ \\
90850770 & 2207.01 & TOI-2207 b & $1.580_{-0.041}^{+0.041}$ & $0.318_{-0.033}^{+0.033}$ & $0.44_{-0.18}^{+0.12}$ & $0.0657_{-0.0019}^{+0.0025}$ & $11.39_{-0.47}^{+0.49}$ & $0.42_{-0.27}^{+0.24}$ & $8.002007_{-0.000017}^{+0.000017}$ & $2043.7686_{-0.0016}^{+0.0016}$ & $0.09_{-0.09}^{+0.25}$ & $180_{-190}^{+0}$ \\
91987762 & 1898.01 & TOI-1898 b & $1.615_{-0.029}^{+0.029}$ & $0.347_{-0.024}^{+0.024}$ & $1.14_{-0.18}^{+0.25}$ & $0.0556_{-0.0009}^{+0.0010}$ & $9.81_{-0.23}^{+0.24}$ & $0.789_{-0.038}^{+0.028}$ & $45.522217_{-0.000095}^{+0.000095}$ & $2531.56400_{-0.00052}^{+0.00052}$ & $0.43_{-0.12}^{+0.22}$ & $30_{-10}^{+140}$ \\
95079513 & 5504.01 &  & $1.191_{-0.030}^{+0.030}$ & $0.614_{-0.084}^{+0.084}$ & $0.50_{-0.39}^{+0.38}$ & $0.0399_{-0.0033}^{+0.0071}$ & $5.50_{-0.76}^{+0.59}$ & $0.57_{-0.38}^{+0.31}$ & $13.2430_{-0.0022}^{+0.0022}$ & $2563.0514_{-0.0049}^{+0.0049}$ & $0.00_{-0.00}^{+0.38}$ & $-150_{-30}^{+160}$ \\
96317115 & 4806.01 &  & $1.152_{-0.030}^{+0.030}$ & $0.687_{-0.098}^{+0.098}$ & $0.53_{-0.37}^{+0.35}$ & $0.0425_{-0.0033}^{+0.0049}$ & $5.48_{-0.54}^{+0.53}$ & $0.53_{-0.36}^{+0.30}$ & $8.44771_{-0.00011}^{+0.00011}$ & $2248.2934_{-0.0048}^{+0.0048}$ & $0.08_{-0.08}^{+0.30}$ & $-140_{-40}^{+140}$ \\
99989903 & 6673.01 &  & $1.431_{-0.028}^{+0.028}$ & $0.394_{-0.041}^{+0.041}$ & $0.23_{-0.18}^{+0.14}$ & $0.0156_{-0.0013}^{+0.0031}$ & $2.62_{-0.40}^{+0.28}$ & $0.53_{-0.36}^{+0.35}$ & $19.74712_{-0.00030}^{+0.00030}$ & $1702.993_{-0.011}^{+0.011}$ & $0.02_{-0.02}^{+0.39}$ & $-150_{-20}^{+130}$ \\
101948569 & 240.01 &  & $0.721_{-0.022}^{+0.022}$ & $1.92_{-0.21}^{+0.21}$ & $1.2_{-1.1}^{+1.3}$ & $0.038_{-0.004}^{+0.017}$ & $3.63_{-0.98}^{+0.68}$ & $0.61_{-0.41}^{+0.35}$ & $19.47230_{-0.00012}^{+0.00012}$ & $1360.1170_{-0.0084}^{+0.0084}$ & $0.16_{-0.16}^{+0.28}$ & $-140_{-40}^{+140}$ \\
103448870 & 1687.01 &  & $0.965_{-0.022}^{+0.022}$ & $1.14_{-0.11}^{+0.11}$ & $15_{-10}^{+8}$ & $0.0319_{-0.0019}^{+0.0027}$ & $3.42_{-0.26}^{+0.23}$ & $0.53_{-0.36}^{+0.30}$ & $10.259641_{-0.000020}^{+0.000020}$ & $1816.8432_{-0.0017}^{+0.0017}$ & $0.73_{-0.08}^{+0.15}$ & $85_{-58}^{+58}$ \\
105840719 & 2123.01 &  & $0.843_{-0.021}^{+0.021}$ & $1.52_{-0.14}^{+0.14}$ & $1.01_{-0.52}^{+0.34}$ & $0.0436_{-0.0017}^{+0.0021}$ & $4.04_{-0.19}^{+0.22}$ & $0.45_{-0.31}^{+0.27}$ & $10.308816_{-0.000040}^{+0.000040}$ & $2691.8171_{-0.0024}^{+0.0024}$ & $0.03_{-0.03}^{+0.34}$ & $-150_{-10}^{+130}$ \\
115524421 & 2064.01 & WASP-148 c & $0.928_{-0.023}^{+0.023}$ & $1.21_{-0.17}^{+0.17}$ & $1.52_{-0.71}^{+0.64}$ & $0.0846_{-0.0042}^{+0.0053}$ & $8.64_{-0.54}^{+0.51}$ & $0.49_{-0.32}^{+0.23}$ & $8.803665_{-0.000031}^{+0.000031}$ & $2735.8521_{-0.0018}^{+0.0018}$ & $0.06_{-0.06}^{+0.28}$ & $-10_{-30}^{+190}$ \\
116382006 & 3977.01 &  & $1.241_{-0.064}^{+0.064}$ & $0.486_{-0.089}^{+0.089}$ & $0.11_{-0.03}^{+0.14}$ & $0.097_{-0.012}^{+0.005}$ & $12.4_{-1.3}^{+1.4}$ & $0.83_{-0.25}^{+0.05}$ & $23.25487_{-0.00011}^{+0.00011}$ & $2679.9428_{-0.0025}^{+0.0025}$ & $0.36_{-0.23}^{+0.33}$ & $-124_{-19}^{+85}$ \\
118406995 & 2912.01 &  & $2.017_{-0.062}^{+0.062}$ & $0.172_{-0.023}^{+0.023}$ & $0.261_{-0.047}^{+0.066}$ & $0.0698_{-0.0019}^{+0.0023}$ & $15.41_{-0.67}^{+0.65}$ & $0.839_{-0.037}^{+0.026}$ & $8.761466_{-0.000014}^{+0.000014}$ & $3019.66182_{-0.00098}^{+0.00098}$ & $0.17_{-0.17}^{+0.20}$ & $0_{-10}^{+170}$ \\
120255950 & 4584.01 & Kepler-1656 c & $1.000_{-0.021}^{+0.021}$ & $1.05_{-0.11}^{+0.11}$ & $14.1_{-8.3}^{+6.7}$ & $0.0444_{-0.0021}^{+0.0026}$ & $4.88_{-0.27}^{+0.28}$ & $0.50_{-0.34}^{+0.27}$ & $31.57883_{-0.00014}^{+0.00014}$ & $2399.6385_{-0.0013}^{+0.0013}$ & $0.76_{-0.11}^{+0.11}$ & $106_{-80}^{+42}$ \\
123357864 & 6005.01 & Kepler-102 f & $0.746_{-0.014}^{+0.014}$ & $1.87_{-0.14}^{+0.14}$ & $1.3_{-1.2}^{+1.9}$ & $0.025_{-0.003}^{+0.010}$ & $2.34_{-0.61}^{+0.48}$ & $0.58_{-0.39}^{+0.38}$ & $16.14601_{-0.00066}^{+0.00066}$ & $1697.389_{-0.034}^{+0.034}$ & $0.03_{-0.03}^{+0.47}$ & $-150_{-30}^{+180}$ \\
124029677 & 5153.01 & TOI-5153 b & $1.441_{-0.040}^{+0.040}$ & $0.465_{-0.050}^{+0.050}$ & $1.32_{-0.46}^{+0.25}$ & $0.0728_{-0.0020}^{+0.0026}$ & $11.49_{-0.50}^{+0.47}$ & $0.35_{-0.24}^{+0.25}$ & $20.910853_{-0.000071}^{+0.000071}$ & $2197.0938_{-0.0015}^{+0.0015}$ & $0.38_{-0.12}^{+0.22}$ & $30_{-10}^{+130}$ \\
126322519 & 5502.01 &  & $1.360_{-0.039}^{+0.039}$ & $0.528_{-0.084}^{+0.084}$ & $1.31_{-0.87}^{+0.61}$ & $0.0298_{-0.0021}^{+0.0035}$ & $4.56_{-0.47}^{+0.41}$ & $0.48_{-0.32}^{+0.32}$ & $11.62599_{-0.00013}^{+0.00013}$ & $2578.3594_{-0.0032}^{+0.0032}$ & $0.35_{-0.23}^{+0.25}$ & $150_{-140}^{+20}$ \\
130924120 & 757.01 & TOI-757 b & $0.767_{-0.019}^{+0.019}$ & $1.82_{-0.17}^{+0.17}$ & $1.05_{-0.83}^{+0.63}$ & $0.0307_{-0.0020}^{+0.0050}$ & $2.73_{-0.33}^{+0.26}$ & $0.51_{-0.35}^{+0.35}$ & $17.468203_{-0.000076}^{+0.000076}$ & $3039.1959_{-0.0035}^{+0.0035}$ & $0.03_{-0.03}^{+0.38}$ & $-40_{-120}^{+20}$ \\
138588540 & 1434.01 &  & $0.762_{-0.016}^{+0.016}$ & $1.66_{-0.11}^{+0.11}$ & $1.6_{-1.1}^{+1.0}$ & $0.0255_{-0.0021}^{+0.0025}$ & $2.14_{-0.20}^{+0.18}$ & $0.50_{-0.34}^{+0.31}$ & $29.87192_{-0.00071}^{+0.00071}$ & $1703.473_{-0.017}^{+0.017}$ & $0.05_{-0.05}^{+0.31}$ & $-150_{-30}^{+160}$ \\
142381532 & 1823.01 & TOI-1823 b & $0.795_{-0.018}^{+0.018}$ & $1.69_{-0.15}^{+0.15}$ & $1.20_{-0.23}^{+0.20}$ & $0.0862_{-0.0017}^{+0.0022}$ & $7.51_{-0.26}^{+0.21}$ & $0.36_{-0.22}^{+0.15}$ & $38.813530_{-0.000061}^{+0.000061}$ & $3345.3486_{-0.0017}^{+0.0017}$ & $0.15_{-0.15}^{+0.18}$ & $-150_{-0}^{+120}$ \\
142387023 & 1824.01 & TOI-1824 b & $0.823_{-0.026}^{+0.026}$ & $1.51_{-0.18}^{+0.18}$ & $1.32_{-0.89}^{+0.71}$ & $0.0306_{-0.0022}^{+0.0029}$ & $2.79_{-0.25}^{+0.23}$ & $0.49_{-0.33}^{+0.31}$ & $22.80852_{-0.00027}^{+0.00027}$ & $3362.101_{-0.011}^{+0.011}$ & $0.02_{-0.02}^{+0.33}$ & $-150_{-30}^{+160}$ \\
142394656 & 1268.01 & TOI-1268 b & $0.882_{-0.019}^{+0.019}$ & $1.34_{-0.12}^{+0.12}$ & $0.95_{-0.15}^{+0.09}$ & $0.0901_{-0.0014}^{+0.0017}$ & $8.69_{-0.24}^{+0.24}$ & $0.27_{-0.18}^{+0.16}$ & $8.1577260_{-0.0000090}^{+0.0000090}$ & $3359.6082_{-0.0014}^{+0.0014}$ & $0.13_{-0.11}^{+0.23}$ & $-30_{-120}^{+10}$ \\
142868621 & 2446.01 &  & $0.992_{-0.023}^{+0.023}$ & $0.90_{-0.16}^{+0.16}$ & $0.64_{-0.56}^{+0.60}$ & $0.0331_{-0.0029}^{+0.0075}$ & $3.90_{-0.67}^{+0.46}$ & $0.60_{-0.41}^{+0.33}$ & $18.6703_{-0.0066}^{+0.0066}$ & $1419.53_{-0.26}^{+0.26}$ & $0.01_{-0.01}^{+0.41}$ & $-30_{-150}^{+30}$ \\
144193715 & 4308.01 & TOI-4308 b & $0.801_{-0.018}^{+0.018}$ & $1.61_{-0.15}^{+0.15}$ & $1.7_{-1.0}^{+0.8}$ & $0.0270_{-0.0017}^{+0.0022}$ & $2.38_{-0.20}^{+0.16}$ & $0.47_{-0.32}^{+0.31}$ & $9.151208_{-0.000038}^{+0.000038}$ & $3163.6730_{-0.0048}^{+0.0048}$ & $0.02_{-0.02}^{+0.31}$ & $-160_{-20}^{+190}$ \\
147951030 & 2067.01 &  & $0.868_{-0.019}^{+0.019}$ & $1.40_{-0.13}^{+0.13}$ & $1.7_{-1.5}^{+1.4}$ & $0.0266_{-0.0026}^{+0.0075}$ & $2.82_{-0.54}^{+0.43}$ & $0.57_{-0.39}^{+0.36}$ & $8.812825_{-0.000069}^{+0.000069}$ & $3366.2139_{-0.0094}^{+0.0094}$ & $0.05_{-0.05}^{+0.36}$ & $-160_{-20}^{+210}$ \\
148782377 & 1415.01 &  & $1.426_{-0.037}^{+0.037}$ & $0.397_{-0.041}^{+0.041}$ & $0.42_{-0.29}^{+0.22}$ & $0.0313_{-0.0012}^{+0.0021}$ & $4.95_{-0.31}^{+0.26}$ & $0.52_{-0.36}^{+0.30}$ & $14.42070_{-0.00026}^{+0.00026}$ & $1933.1776_{-0.0026}^{+0.0026}$ & $0.04_{-0.04}^{+0.30}$ & $-160_{-20}^{+190}$ \\
150098860 & 220.01 & TOI-220 b & $0.858_{-0.025}^{+0.025}$ & $1.39_{-0.16}^{+0.16}$ & $1.6_{-0.9}^{+4.4}$ & $0.0294_{-0.0030}^{+0.0021}$ & $2.69_{-0.23}^{+0.28}$ & $0.80_{-0.51}^{+0.09}$ & $10.695299_{-0.000012}^{+0.000012}$ & $3175.4935_{-0.0012}^{+0.0012}$ & $0.02_{-0.02}^{+0.48}$ & $-40_{-140}^{+90}$ \\
154089169 & 1174.01 & TOI-1174 b & $0.761_{-0.014}^{+0.014}$ & $1.87_{-0.16}^{+0.16}$ & $1.43_{-0.99}^{+0.69}$ & $0.0301_{-0.0020}^{+0.0032}$ & $2.57_{-0.25}^{+0.20}$ & $0.49_{-0.33}^{+0.33}$ & $8.953451_{-0.000049}^{+0.000049}$ & $3355.4000_{-0.0077}^{+0.0077}$ & $0.04_{-0.04}^{+0.32}$ & $-150_{-20}^{+140}$ \\
154474036 & 4578.01 &  & $0.905_{-0.019}^{+0.019}$ & $1.29_{-0.12}^{+0.12}$ & $2.5_{-2.3}^{+2.0}$ & $0.0232_{-0.0023}^{+0.0073}$ & $2.62_{-0.53}^{+0.41}$ & $0.56_{-0.38}^{+0.38}$ & $8.623903_{-0.000073}^{+0.000073}$ & $2634.1968_{-0.0046}^{+0.0046}$ & $0.11_{-0.11}^{+0.38}$ & $180_{-200}^{+0}$ \\
154716798 & 1239.01 &  & $0.784_{-0.021}^{+0.021}$ & $1.75_{-0.18}^{+0.18}$ & $1.69_{-0.80}^{+0.53}$ & $0.0552_{-0.0025}^{+0.0028}$ & $4.74_{-0.26}^{+0.25}$ & $0.42_{-0.29}^{+0.27}$ & $12.639699_{-0.000053}^{+0.000053}$ & $2604.0954_{-0.0017}^{+0.0017}$ & $0.00_{-0.00}^{+0.30}$ & $-20_{-160}^{+30}$ \\
154741689 & 2170.01 &  & $1.118_{-0.025}^{+0.025}$ & $0.719_{-0.097}^{+0.097}$ & $0.22_{-0.20}^{+0.17}$ & $0.0225_{-0.0021}^{+0.0072}$ & $3.14_{-0.65}^{+0.50}$ & $0.58_{-0.40}^{+0.36}$ & $9.27857_{-0.00018}^{+0.00018}$ & $3469.238_{-0.016}^{+0.016}$ & $0.44_{-0.35}^{+0.18}$ & $-49_{-95}^{+11}$ \\
154872375 & 1135.01 & TOI-1135 b & $1.171_{-0.028}^{+0.028}$ & $0.723_{-0.097}^{+0.097}$ & $0.61_{-0.10}^{+0.06}$ & $0.06938_{-0.00081}^{+0.00088}$ & $8.87_{-0.25}^{+0.22}$ & $0.27_{-0.18}^{+0.16}$ & $8.0277280_{-0.0000060}^{+0.0000060}$ & $3466.30837_{-0.00079}^{+0.00079}$ & $0.00_{-0.00}^{+0.26}$ & $-150_{-10}^{+140}$ \\
157667414 & 4576.01 &  & $0.628_{-0.015}^{+0.015}$ & $2.65_{-0.23}^{+0.23}$ & $1.7_{-1.5}^{+2.5}$ & $0.0308_{-0.0054}^{+0.0079}$ & $2.21_{-0.44}^{+0.46}$ & $0.55_{-0.37}^{+0.37}$ & $10.48336_{-0.00065}^{+0.00065}$ & $2010.848_{-0.028}^{+0.028}$ & $0.50_{-0.50}^{+0.50}$ & $180_{-180}^{+180}$ \\
158002130 & 1180.01 & TOI-1180 b & $0.709_{-0.015}^{+0.015}$ & $2.11_{-0.17}^{+0.17}$ & $2.0_{-1.1}^{+1.0}$ & $0.0373_{-0.0015}^{+0.0022}$ & $2.92_{-0.16}^{+0.15}$ & $0.52_{-0.34}^{+0.25}$ & $9.686751_{-0.000016}^{+0.000016}$ & $3473.4114_{-0.0022}^{+0.0022}$ & $0.03_{-0.03}^{+0.29}$ & $-150_{-30}^{+170}$ \\
160039081 & 2082.01 &  & $1.196_{-0.023}^{+0.023}$ & $0.58_{-0.11}^{+0.11}$ & $1.00_{-0.81}^{+0.77}$ & $0.0223_{-0.0012}^{+0.0029}$ & $3.05_{-0.29}^{+0.24}$ & $0.59_{-0.39}^{+0.30}$ & $30.20059_{-0.00015}^{+0.00015}$ & $3444.1547_{-0.0051}^{+0.0051}$ & $0.07_{-0.07}^{+0.38}$ & $-170_{-150}^{+350}$ \\
165527918 & 2101.01 &  & $0.996_{-0.024}^{+0.024}$ & $0.87_{-0.12}^{+0.12}$ & $0.65_{-0.50}^{+0.46}$ & $0.0244_{-0.0014}^{+0.0030}$ & $2.76_{-0.26}^{+0.23}$ & $0.57_{-0.38}^{+0.30}$ & $9.075280_{-0.000034}^{+0.000034}$ & $1690.4247_{-0.0033}^{+0.0033}$ & $0.09_{-0.09}^{+0.29}$ & $-150_{-20}^{+160}$ \\
165763244 & 1805.01 &  & $0.840_{-0.021}^{+0.021}$ & $1.48_{-0.15}^{+0.15}$ & $1.9_{-1.4}^{+1.2}$ & $0.0345_{-0.0027}^{+0.0056}$ & $3.33_{-0.41}^{+0.35}$ & $0.52_{-0.35}^{+0.33}$ & $24.05126_{-0.00018}^{+0.00018}$ & $2671.1515_{-0.0047}^{+0.0047}$ & $0.12_{-0.12}^{+0.27}$ & $-20_{-20}^{+200}$ \\
166739520 & 190.01 & WASP-117 b & $1.233_{-0.026}^{+0.026}$ & $0.553_{-0.091}^{+0.091}$ & $0.299_{-0.019}^{+0.023}$ & $0.08665_{-0.00071}^{+0.00064}$ & $11.65_{-0.24}^{+0.28}$ & $0.434_{-0.057}^{+0.043}$ & $10.0205880_{-0.0000030}^{+0.0000030}$ & $2139.17818_{-0.00016}^{+0.00016}$ & $0.24_{-0.12}^{+0.23}$ & $-142_{-8}^{+93}$ \\
167661160 & 2479.01 &  & $0.992_{-0.022}^{+0.022}$ & $1.082_{-0.091}^{+0.091}$ & $1.32_{-0.66}^{+0.40}$ & $0.0292_{-0.0015}^{+0.0021}$ & $3.19_{-0.22}^{+0.19}$ & $0.41_{-0.28}^{+0.28}$ & $36.83861_{-0.00032}^{+0.00032}$ & $1442.0713_{-0.0030}^{+0.0030}$ & $0.00_{-0.00}^{+0.32}$ & $-170_{-140}^{+350}$ \\
169191182 & 6414.01 &  & $1.321_{-0.034}^{+0.034}$ & $0.538_{-0.053}^{+0.053}$ & $0.74_{-0.40}^{+0.28}$ & $0.0373_{-0.0019}^{+0.0029}$ & $5.47_{-0.41}^{+0.34}$ & $0.45_{-0.30}^{+0.28}$ & $17.760750_{-0.000067}^{+0.000067}$ & $2987.7312_{-0.0030}^{+0.0030}$ & $0.00_{-0.00}^{+0.36}$ & $-10_{-10}^{+190}$ \\
175193677 & 5140.01 & HD 73344 d & $1.208_{-0.031}^{+0.031}$ & $0.616_{-0.077}^{+0.077}$ & $1.7_{-1.2}^{+1.0}$ & $0.0210_{-0.0012}^{+0.0020}$ & $2.84_{-0.22}^{+0.22}$ & $0.54_{-0.36}^{+0.31}$ & $15.6101_{-0.0026}^{+0.0026}$ & $2547.7227_{-0.0020}^{+0.0020}$ & $0.42_{-0.25}^{+0.24}$ & $10_{-10}^{+150}$ \\
177162886 & 899.01 &  & $1.133_{-0.028}^{+0.028}$ & $0.73_{-0.11}^{+0.11}$ & $1.33_{-0.20}^{+0.21}$ & $0.0887_{-0.0018}^{+0.0021}$ & $10.98_{-0.34}^{+0.36}$ & $0.715_{-0.046}^{+0.047}$ & $12.8461880_{-0.0000050}^{+0.0000050}$ & $1544.86908_{-0.00034}^{+0.00034}$ & $0.26_{-0.15}^{+0.21}$ & $170_{-150}^{+10}$ \\
179739873 & 6556.01 &  & $1.371_{-0.032}^{+0.032}$ & $0.445_{-0.066}^{+0.066}$ & $0.61_{-0.50}^{+0.51}$ & $0.0437_{-0.0038}^{+0.0083}$ & $7.0_{-1.0}^{+0.8}$ & $0.58_{-0.39}^{+0.32}$ & $12.96234_{-0.00054}^{+0.00054}$ & $3085.1702_{-0.0047}^{+0.0047}$ & $0.05_{-0.05}^{+0.37}$ & $-170_{-130}^{+350}$ \\
180931993 & 6468.01 &  & $1.522_{-0.045}^{+0.045}$ & $0.375_{-0.045}^{+0.045}$ & $0.57_{-0.27}^{+0.18}$ & $0.0752_{-0.0044}^{+0.0044}$ & $12.51_{-0.82}^{+0.78}$ & $0.38_{-0.26}^{+0.29}$ & $12.12266_{-0.00029}^{+0.00029}$ & $3007.9707_{-0.0038}^{+0.0038}$ & $0.02_{-0.02}^{+0.36}$ & $-10_{-20}^{+170}$ \\
182078202 & 4302.01 &  & $0.889_{-0.021}^{+0.021}$ & $1.20_{-0.16}^{+0.16}$ & $1.5_{-1.2}^{+0.9}$ & $0.0265_{-0.0018}^{+0.0035}$ & $2.67_{-0.28}^{+0.25}$ & $0.52_{-0.35}^{+0.34}$ & $38.76194_{-0.00021}^{+0.00021}$ & $1347.7643_{-0.0061}^{+0.0061}$ & $0.01_{-0.01}^{+0.38}$ & $-20_{-20}^{+200}$ \\
183532609 & 191.01 & WASP-8 c & $1.031_{-0.046}^{+0.046}$ & $0.82_{-0.15}^{+0.15}$ & $0.444_{-0.039}^{+0.047}$ & $0.1142_{-0.0020}^{+0.0018}$ & $12.81_{-0.57}^{+0.64}$ & $0.629_{-0.047}^{+0.035}$ & $8.1587250_{-0.0000040}^{+0.0000040}$ & $3202.79283_{-0.00047}^{+0.00047}$ & $0.23_{-0.13}^{+0.24}$ & $-38_{-99}^{+5}$ \\
192790476 & 2459.01 & TOI-2459 b & $0.639_{-0.019}^{+0.019}$ & $2.48_{-0.25}^{+0.25}$ & $2.2_{-1.6}^{+1.7}$ & $0.0383_{-0.0035}^{+0.0050}$ & $2.74_{-0.31}^{+0.29}$ & $0.53_{-0.36}^{+0.32}$ & $19.10471_{-0.00021}^{+0.00021}$ & $1452.3355_{-0.0048}^{+0.0048}$ & $0.07_{-0.07}^{+0.31}$ & $-30_{-150}^{+50}$ \\
192988021 & 2808.01 &  & $0.684_{-0.015}^{+0.015}$ & $2.21_{-0.20}^{+0.20}$ & $1.4_{-1.1}^{+1.0}$ & $0.0263_{-0.0022}^{+0.0047}$ & $2.08_{-0.27}^{+0.24}$ & $0.57_{-0.38}^{+0.33}$ & $9.445374_{-0.000050}^{+0.000050}$ & $3000.0578_{-0.0050}^{+0.0050}$ & $0.03_{-0.03}^{+0.38}$ & $-40_{-130}^{+30}$ \\
193220940 & 2806.01 &  & $1.428_{-0.036}^{+0.036}$ & $0.400_{-0.054}^{+0.054}$ & $0.78_{-0.38}^{+0.20}$ & $0.0300_{-0.0012}^{+0.0014}$ & $4.69_{-0.25}^{+0.21}$ & $0.38_{-0.26}^{+0.29}$ & $11.404617_{-0.000049}^{+0.000049}$ & $2298.6228_{-0.0021}^{+0.0021}$ & $0.23_{-0.16}^{+0.27}$ & $10_{-10}^{+150}$ \\
197598125 & 6825.01 &  & $1.023_{-0.027}^{+0.027}$ & $0.89_{-0.12}^{+0.12}$ & $0.42_{-0.37}^{+0.41}$ & $0.044_{-0.004}^{+0.019}$ & $6.0_{-1.5}^{+1.1}$ & $0.60_{-0.41}^{+0.35}$ & $16.45467_{-0.00023}^{+0.00023}$ & $3170.126_{-0.012}^{+0.012}$ & $0.18_{-0.18}^{+0.28}$ & $-50_{-120}^{+30}$ \\
198356533 & 1437.01 & TOI-1437 b & $1.263_{-0.025}^{+0.025}$ & $0.510_{-0.070}^{+0.070}$ & $0.38_{-0.22}^{+0.11}$ & $0.0178_{-0.0005}^{+0.0012}$ & $2.51_{-0.14}^{+0.12}$ & $0.42_{-0.28}^{+0.32}$ & $18.840917_{-0.000060}^{+0.000060}$ & $2906.5504_{-0.0019}^{+0.0019}$ & $0.00_{-0.00}^{+0.33}$ & $-30_{-140}^{+20}$ \\
199376584 & 1456.01 & HD 332231 b & $1.282_{-0.040}^{+0.040}$ & $0.529_{-0.073}^{+0.073}$ & $0.247_{-0.016}^{+0.019}$ & $0.07319_{-0.00070}^{+0.00081}$ & $10.25_{-0.32}^{+0.35}$ & $0.675_{-0.024}^{+0.020}$ & $18.711693_{-0.000015}^{+0.000015}$ & $3544.72314_{-0.00092}^{+0.00092}$ & $0.27_{-0.09}^{+0.24}$ & $-40_{-86}^{+5}$ \\
203377303 & 3493.01 &  & $1.225_{-0.025}^{+0.025}$ & $0.551_{-0.075}^{+0.075}$ & $0.43_{-0.25}^{+0.15}$ & $0.0259_{-0.0011}^{+0.0022}$ & $3.55_{-0.25}^{+0.21}$ & $0.45_{-0.30}^{+0.31}$ & $8.159466_{-0.000071}^{+0.000071}$ & $2313.0446_{-0.0062}^{+0.0062}$ & $0.01_{-0.01}^{+0.32}$ & $-30_{-150}^{+20}$ \\
204671232 & 2361.01 &  & $1.036_{-0.029}^{+0.029}$ & $0.94_{-0.11}^{+0.11}$ & $0.98_{-0.17}^{+0.09}$ & $0.1043_{-0.0019}^{+0.0021}$ & $11.80_{-0.39}^{+0.38}$ & $0.24_{-0.16}^{+0.19}$ & $8.733509_{-0.000010}^{+0.000010}$ & $1577.7438_{-0.0012}^{+0.0012}$ & $0.00_{-0.00}^{+0.22}$ & $-170_{-10}^{+190}$ \\
206541859 & 4406.01 & TOI-4406 b & $1.338_{-0.029}^{+0.029}$ & $0.476_{-0.063}^{+0.063}$ & $0.65_{-0.07}^{+0.10}$ & $0.0784_{-0.0027}^{+0.0033}$ & $11.49_{-0.45}^{+0.56}$ & $0.893_{-0.018}^{+0.012}$ & $30.083553_{-0.000037}^{+0.000037}$ & $2064.11782_{-0.00082}^{+0.00082}$ & $0.10_{-0.10}^{+0.24}$ & $-10_{-0}^{+190}$ \\
207110080 & 558.01 & TOI-558 b & $1.565_{-0.034}^{+0.034}$ & $0.307_{-0.033}^{+0.033}$ & $2.2_{-1.3}^{+3.9}$ & $0.071_{-0.014}^{+0.009}$ & $11.5_{-1.8}^{+2.2}$ & $0.74_{-0.52}^{+0.16}$ & $14.574043_{-0.000037}^{+0.000037}$ & $2133.40658_{-0.00097}^{+0.00097}$ & $0.62_{-0.18}^{+0.30}$ & $77_{-55}^{+91}$ \\
219436394 & 2100.01 &  & $0.856_{-0.019}^{+0.019}$ & $1.50_{-0.14}^{+0.14}$ & $7.7_{-5.1}^{+4.0}$ & $0.0321_{-0.0021}^{+0.0029}$ & $3.04_{-0.26}^{+0.23}$ & $0.48_{-0.33}^{+0.32}$ & $23.65737_{-0.00014}^{+0.00014}$ & $2605.6410_{-0.0027}^{+0.0027}$ & $0.57_{-0.18}^{+0.19}$ & $95_{-77}^{+57}$ \\
219857012 & 1742.01 & TOI-1742 b & $1.158_{-0.027}^{+0.027}$ & $0.633_{-0.095}^{+0.095}$ & $0.21_{-0.14}^{+0.30}$ & $0.0197_{-0.0009}^{+0.0013}$ & $2.51_{-0.15}^{+0.14}$ & $0.70_{-0.45}^{+0.17}$ & $21.26863_{-0.00016}^{+0.00016}$ & $3533.2051_{-0.0060}^{+0.0060}$ & $0.14_{-0.13}^{+0.38}$ & $-130_{-20}^{+110}$ \\
219978369 & 6785.01 &  & $1.675_{-0.050}^{+0.050}$ & $0.239_{-0.034}^{+0.034}$ & $0.196_{-0.077}^{+0.041}$ & $0.0526_{-0.0021}^{+0.0022}$ & $9.61_{-0.47}^{+0.48}$ & $0.35_{-0.24}^{+0.27}$ & $16.250196_{-0.000095}^{+0.000095}$ & $3129.5176_{-0.0059}^{+0.0059}$ & $0.00_{-0.00}^{+0.29}$ & $-30_{-140}^{+20}$ \\
224297408 & 5733.01 &  & $0.733_{-0.017}^{+0.017}$ & $1.93_{-0.18}^{+0.18}$ & $3.3_{-3.0}^{+3.3}$ & $0.0293_{-0.0037}^{+0.0083}$ & $2.57_{-0.54}^{+0.42}$ & $0.55_{-0.37}^{+0.38}$ & $8.27515_{-0.00011}^{+0.00011}$ & $1711.6050_{-0.0064}^{+0.0064}$ & $0.13_{-0.13}^{+0.37}$ & $-170_{-130}^{+350}$ \\
224299081 & 5619.01 &  & $1.360_{-0.036}^{+0.036}$ & $0.395_{-0.067}^{+0.067}$ & $0.93_{-0.42}^{+0.26}$ & $0.0524_{-0.0018}^{+0.0024}$ & $7.83_{-0.36}^{+0.38}$ & $0.41_{-0.28}^{+0.26}$ & $37.99839_{-0.00022}^{+0.00022}$ & $2626.9007_{-0.0030}^{+0.0030}$ & $0.33_{-0.16}^{+0.25}$ & $150_{-130}^{+20}$ \\
224328450 & 5699.01 &  & $1.692_{-0.039}^{+0.039}$ & $0.233_{-0.036}^{+0.036}$ & $1.7_{-1.2}^{+1.2}$ & $0.0582_{-0.0049}^{+0.0082}$ & $11.1_{-1.4}^{+1.1}$ & $0.55_{-0.37}^{+0.30}$ & $22.01841_{-0.00073}^{+0.00073}$ & $2704.1503_{-0.0035}^{+0.0035}$ & $0.63_{-0.13}^{+0.21}$ & $92_{-75}^{+52}$ \\
224596152 & 1734.01 &  & $1.002_{-0.021}^{+0.021}$ & $1.05_{-0.12}^{+0.12}$ & $1.4_{-1.0}^{+0.8}$ & $0.0237_{-0.0014}^{+0.0023}$ & $2.64_{-0.22}^{+0.19}$ & $0.51_{-0.35}^{+0.32}$ & $28.87445_{-0.00021}^{+0.00021}$ & $1688.8671_{-0.0056}^{+0.0056}$ & $0.10_{-0.10}^{+0.28}$ & $-10_{-30}^{+190}$ \\
229786610 & 4113.01 &  & $0.805_{-0.022}^{+0.022}$ & $1.66_{-0.16}^{+0.16}$ & $2.4_{-1.4}^{+0.9}$ & $0.0268_{-0.0016}^{+0.0020}$ & $2.37_{-0.17}^{+0.16}$ & $0.44_{-0.30}^{+0.30}$ & $22.15755_{-0.00010}^{+0.00010}$ & $2839.0749_{-0.0038}^{+0.0038}$ & $0.08_{-0.08}^{+0.29}$ & $-10_{-10}^{+190}$ \\
229944666 & 1464.01 &  & $0.966_{-0.027}^{+0.027}$ & $0.96_{-0.10}^{+0.10}$ & $2.7_{-1.9}^{+1.5}$ & $0.0266_{-0.0016}^{+0.0026}$ & $2.86_{-0.25}^{+0.22}$ & $0.52_{-0.35}^{+0.31}$ & $11.312517_{-0.000051}^{+0.000051}$ & $2643.7167_{-0.0022}^{+0.0022}$ & $0.38_{-0.18}^{+0.31}$ & $30_{-10}^{+150}$ \\
230017324 & 1280.01 &  & $0.729_{-0.025}^{+0.025}$ & $2.00_{-0.25}^{+0.25}$ & $1.81_{-0.79}^{+0.48}$ & $0.0263_{-0.0007}^{+0.0012}$ & $2.11_{-0.10}^{+0.11}$ & $0.40_{-0.27}^{+0.26}$ & $9.692633_{-0.000015}^{+0.000015}$ & $2757.49296_{-0.00077}^{+0.00077}$ & $0.02_{-0.02}^{+0.27}$ & $-160_{-20}^{+160}$ \\
232540264 & 1247.01 & HD 135694 b & $1.084_{-0.020}^{+0.020}$ & $0.738_{-0.095}^{+0.095}$ & $0.88_{-0.40}^{+0.27}$ & $0.02236_{-0.00054}^{+0.00078}$ & $2.663_{-0.098}^{+0.083}$ & $0.43_{-0.29}^{+0.24}$ & $15.923476_{-0.000025}^{+0.000025}$ & $3311.8424_{-0.0015}^{+0.0015}$ & $0.05_{-0.05}^{+0.26}$ & $-20_{-20}^{+200}$ \\
232976128 & 1249.01 & TOI-1249 b & $0.991_{-0.024}^{+0.024}$ & $0.88_{-0.16}^{+0.16}$ & $1.3_{-1.0}^{+1.2}$ & $0.0312_{-0.0025}^{+0.0044}$ & $3.50_{-0.42}^{+0.34}$ & $0.63_{-0.42}^{+0.26}$ & $13.079127_{-0.000076}^{+0.000076}$ & $3342.3491_{-0.0073}^{+0.0073}$ & $0.05_{-0.05}^{+0.38}$ & $-20_{-20}^{+200}$ \\
232982938 & 1828.01 &  & $1.580_{-0.038}^{+0.038}$ & $0.272_{-0.040}^{+0.040}$ & $0.51_{-0.15}^{+0.05}$ & $0.0500_{-0.0008}^{+0.0014}$ & $8.69_{-0.28}^{+0.28}$ & $0.28_{-0.19}^{+0.25}$ & $9.094105_{-0.000011}^{+0.000011}$ & $2918.44016_{-0.00077}^{+0.00077}$ & $0.25_{-0.14}^{+0.24}$ & $10_{-10}^{+170}$ \\
233633993 & 2083.01 &  & $0.723_{-0.019}^{+0.019}$ & $2.01_{-0.19}^{+0.19}$ & $0.82_{-0.63}^{+0.66}$ & $0.0329_{-0.0029}^{+0.0056}$ & $2.73_{-0.40}^{+0.27}$ & $0.57_{-0.38}^{+0.31}$ & $17.96956_{-0.00015}^{+0.00015}$ & $1695.8743_{-0.0080}^{+0.0080}$ & $0.16_{-0.16}^{+0.32}$ & $-40_{-110}^{+10}$ \\
235902467 & 4103.01 &  & $1.042_{-0.027}^{+0.027}$ & $0.92_{-0.11}^{+0.11}$ & $1.37_{-0.16}^{+0.17}$ & $0.1086_{-0.0022}^{+0.0024}$ & $12.35_{-0.44}^{+0.36}$ & $0.485_{-0.082}^{+0.072}$ & $12.2740760_{-0.0000060}^{+0.0000060}$ & $2754.90280_{-0.00030}^{+0.00030}$ & $0.16_{-0.10}^{+0.24}$ & $0_{-0}^{+160}$ \\
237015185 & 5604.01 &  & $1.456_{-0.038}^{+0.038}$ & $0.437_{-0.050}^{+0.050}$ & $0.56_{-0.30}^{+0.19}$ & $0.0481_{-0.0023}^{+0.0028}$ & $7.71_{-0.47}^{+0.42}$ & $0.42_{-0.28}^{+0.29}$ & $11.180146_{-0.000094}^{+0.000094}$ & $2840.5753_{-0.0028}^{+0.0028}$ & $0.06_{-0.06}^{+0.29}$ & $-160_{-140}^{+340}$ \\
237099296 & 1750.01 &  & $0.762_{-0.015}^{+0.015}$ & $1.76_{-0.16}^{+0.16}$ & $1.8_{-1.3}^{+0.9}$ & $0.0326_{-0.0021}^{+0.0050}$ & $2.87_{-0.34}^{+0.27}$ & $0.50_{-0.34}^{+0.32}$ & $11.337280_{-0.000042}^{+0.000042}$ & $2663.8305_{-0.0017}^{+0.0017}$ & $0.08_{-0.08}^{+0.27}$ & $-160_{-20}^{+190}$ \\
237222864 & 1255.01 & HIP 97166 c & $0.836_{-0.022}^{+0.022}$ & $1.53_{-0.18}^{+0.18}$ & $12.3_{-6.9}^{+5.2}$ & $0.0270_{-0.0010}^{+0.0019}$ & $2.52_{-0.15}^{+0.15}$ & $0.49_{-0.32}^{+0.26}$ & $10.2888900_{-0.0000080}^{+0.0000080}$ & $3337.87680_{-0.00085}^{+0.00085}$ & $0.66_{-0.13}^{+0.14}$ & $77_{-49}^{+73}$ \\
237232044 & 1443.01 & TOI-1443 b & $0.768_{-0.018}^{+0.018}$ & $1.83_{-0.17}^{+0.17}$ & $1.50_{-0.70}^{+0.44}$ & $0.0284_{-0.0010}^{+0.0013}$ & $2.40_{-0.11}^{+0.11}$ & $0.42_{-0.28}^{+0.26}$ & $23.540701_{-0.000057}^{+0.000057}$ & $3482.3387_{-0.0026}^{+0.0026}$ & $0.03_{-0.03}^{+0.28}$ & $-30_{-140}^{+20}$ \\
237929468 & 4940.01 &  & $1.173_{-0.034}^{+0.034}$ & $0.599_{-0.081}^{+0.081}$ & $0.7_{-0.4}^{+1.4}$ & $0.0505_{-0.0053}^{+0.0043}$ & $6.38_{-0.58}^{+0.68}$ & $0.77_{-0.43}^{+0.12}$ & $25.867803_{-0.000077}^{+0.000077}$ & $2963.7356_{-0.0030}^{+0.0030}$ & $0.02_{-0.02}^{+0.46}$ & $-20_{-160}^{+70}$ \\
238854767 & 4653.01 &  & $1.289_{-0.037}^{+0.037}$ & $0.603_{-0.074}^{+0.074}$ & $0.38_{-0.33}^{+0.27}$ & $0.0327_{-0.0029}^{+0.0079}$ & $5.06_{-0.89}^{+0.66}$ & $0.53_{-0.36}^{+0.38}$ & $16.37604_{-0.00022}^{+0.00022}$ & $3128.436_{-0.016}^{+0.016}$ & $0.03_{-0.03}^{+0.38}$ & $-30_{-140}^{+20}$ \\
240823272 & 3693.01 & TOI-3693 b & $0.776_{-0.023}^{+0.023}$ & $1.83_{-0.21}^{+0.21}$ & $1.58_{-0.30}^{+0.18}$ & $0.1327_{-0.0030}^{+0.0035}$ & $11.25_{-0.44}^{+0.42}$ & $0.28_{-0.19}^{+0.18}$ & $9.088492_{-0.000025}^{+0.000025}$ & $2888.21292_{-0.00056}^{+0.00056}$ & $0.02_{-0.02}^{+0.23}$ & $-160_{-10}^{+140}$ \\
243200602 & 826.01 & WASP-130 b & $1.034_{-0.026}^{+0.026}$ & $0.79_{-0.11}^{+0.11}$ & $1.66_{-0.20}^{+0.10}$ & $0.0921_{-0.0010}^{+0.0014}$ & $10.42_{-0.28}^{+0.29}$ & $0.21_{-0.14}^{+0.15}$ & $11.5509670_{-0.0000050}^{+0.0000050}$ & $3063.00773_{-0.00042}^{+0.00042}$ & $0.29_{-0.10}^{+0.22}$ & $10_{-10}^{+140}$ \\
243244680 & 5065.01 & EPIC 211945201 b & $1.389_{-0.030}^{+0.030}$ & $0.445_{-0.038}^{+0.038}$ & $1.3_{-0.9}^{+1.1}$ & $0.0391_{-0.0031}^{+0.0054}$ & $6.15_{-0.70}^{+0.63}$ & $0.60_{-0.39}^{+0.24}$ & $19.492149_{-0.000046}^{+0.000046}$ & $2575.8509_{-0.0016}^{+0.0016}$ & $0.41_{-0.22}^{+0.28}$ & $160_{-160}^{+0}$ \\
252912175 & 3797.01 &  & $1.264_{-0.042}^{+0.042}$ & $0.487_{-0.084}^{+0.084}$ & $1.6_{-0.8}^{+1.8}$ & $0.0869_{-0.0083}^{+0.0090}$ & $12.0_{-1.4}^{+1.1}$ & $0.69_{-0.38}^{+0.15}$ & $17.62291_{-0.00010}^{+0.00010}$ & $2586.2423_{-0.0036}^{+0.0036}$ & $0.45_{-0.26}^{+0.27}$ & $30_{-20}^{+150}$ \\
254142310 & 3281.01 &  & $1.957_{-0.072}^{+0.072}$ & $0.187_{-0.036}^{+0.036}$ & $0.28_{-0.12}^{+0.06}$ & $0.0538_{-0.0018}^{+0.0021}$ & $11.52_{-0.61}^{+0.58}$ & $0.37_{-0.26}^{+0.27}$ & $9.310840_{-0.000028}^{+0.000028}$ & $2052.4224_{-0.0028}^{+0.0028}$ & $0.10_{-0.10}^{+0.27}$ & $-170_{-170}^{+350}$ \\
259230140 & 4384.01 &  & $1.681_{-0.046}^{+0.046}$ & $0.307_{-0.045}^{+0.045}$ & $0.52_{-0.11}^{+0.05}$ & $0.03662_{-0.00077}^{+0.00075}$ & $6.72_{-0.24}^{+0.21}$ & $0.24_{-0.17}^{+0.20}$ & $14.317104_{-0.000043}^{+0.000043}$ & $3070.24901_{-0.00095}^{+0.00095}$ & $0.21_{-0.12}^{+0.24}$ & $170_{-160}^{+10}$ \\
260367888 & 3354.01 &  & $1.667_{-0.036}^{+0.036}$ & $0.247_{-0.031}^{+0.031}$ & $0.81_{-0.48}^{+0.35}$ & $0.0329_{-0.0015}^{+0.0024}$ & $6.10_{-0.39}^{+0.35}$ & $0.49_{-0.33}^{+0.28}$ & $46.38087_{-0.00020}^{+0.00020}$ & $2983.7517_{-0.0036}^{+0.0036}$ & $0.40_{-0.15}^{+0.26}$ & $130_{-120}^{+30}$ \\
262746281 & 603.01 &  & $1.604_{-0.035}^{+0.035}$ & $0.293_{-0.051}^{+0.051}$ & $0.14_{-0.07}^{+0.16}$ & $0.0479_{-0.0028}^{+0.0028}$ & $8.38_{-0.53}^{+0.52}$ & $0.68_{-0.35}^{+0.13}$ & $16.179768_{-0.000051}^{+0.000051}$ & $3271.2121_{-0.0035}^{+0.0035}$ & $0.00_{-0.00}^{+0.43}$ & $-50_{-110}^{+30}$ \\
263003176 & 130.01 & HD 5278 c & $1.212_{-0.030}^{+0.030}$ & $0.693_{-0.059}^{+0.059}$ & $0.71_{-0.40}^{+0.18}$ & $0.01877_{-0.00040}^{+0.00071}$ & $2.51_{-0.10}^{+0.09}$ & $0.39_{-0.27}^{+0.32}$ & $14.339177_{-0.000014}^{+0.000014}$ & $1336.5596_{-0.0011}^{+0.0011}$ & $0.01_{-0.01}^{+0.30}$ & $-160_{-20}^{+180}$ \\
264678534 & 1611.01 & HD 207897 b & $0.756_{-0.023}^{+0.023}$ & $1.87_{-0.22}^{+0.22}$ & $2.0_{-1.3}^{+1.7}$ & $0.0276_{-0.0014}^{+0.0029}$ & $2.36_{-0.22}^{+0.17}$ & $0.61_{-0.40}^{+0.24}$ & $16.201719_{-0.000018}^{+0.000018}$ & $3449.07026_{-0.00098}^{+0.00098}$ & $0.03_{-0.03}^{+0.35}$ & $-30_{-150}^{+70}$ \\
266593143 & 1283.01 & HAT-P-17 c & $0.865_{-0.021}^{+0.021}$ & $1.39_{-0.14}^{+0.14}$ & $1.195_{-0.079}^{+0.076}$ & $0.1177_{-0.0013}^{+0.0013}$ & $11.11_{-0.29}^{+0.32}$ & $0.26_{-0.13}^{+0.08}$ & $10.3385280_{-0.0000030}^{+0.0000030}$ & $3539.05660_{-0.00033}^{+0.00033}$ & $0.06_{-0.06}^{+0.17}$ & $-160_{-10}^{+140}$ \\
268334473 & 1691.01 & TOI-1691 b & $0.993_{-0.021}^{+0.021}$ & $0.90_{-0.15}^{+0.15}$ & $0.66_{-0.32}^{+0.20}$ & $0.0330_{-0.0008}^{+0.0014}$ & $3.63_{-0.15}^{+0.14}$ & $0.43_{-0.29}^{+0.27}$ & $16.736931_{-0.000030}^{+0.000030}$ & $3458.3090_{-0.0020}^{+0.0020}$ & $0.01_{-0.01}^{+0.32}$ & $-30_{-130}^{+20}$ \\
269838674 & 5413.01 &  & $1.323_{-0.054}^{+0.054}$ & $0.513_{-0.079}^{+0.079}$ & $1.04_{-0.63}^{+0.49}$ & $0.0415_{-0.0028}^{+0.0040}$ & $6.08_{-0.52}^{+0.56}$ & $0.48_{-0.32}^{+0.30}$ & $12.6123_{-0.0017}^{+0.0017}$ & $2534.9208_{-0.0037}^{+0.0037}$ & $0.34_{-0.33}^{+0.14}$ & $180_{-170}^{+0}$ \\
271478281 & 2194.01 & TOI-2194 b & $0.676_{-0.019}^{+0.019}$ & $2.22_{-0.23}^{+0.23}$ & $2.0_{-1.3}^{+1.1}$ & $0.0275_{-0.0013}^{+0.0025}$ & $2.09_{-0.18}^{+0.13}$ & $0.52_{-0.35}^{+0.29}$ & $15.341985_{-0.000052}^{+0.000052}$ & $3141.9859_{-0.0016}^{+0.0016}$ & $0.01_{-0.01}^{+0.34}$ & $-150_{-30}^{+160}$ \\
274151135 & 1105.01 &  & $0.724_{-0.018}^{+0.018}$ & $1.96_{-0.19}^{+0.19}$ & $2.0_{-1.8}^{+2.0}$ & $0.0353_{-0.0032}^{+0.0090}$ & $3.09_{-0.56}^{+0.42}$ & $0.61_{-0.41}^{+0.32}$ & $10.867921_{-0.000063}^{+0.000063}$ & $3086.9735_{-0.0046}^{+0.0046}$ & $0.02_{-0.02}^{+0.39}$ & $-30_{-150}^{+60}$ \\
277128619 & 4994.01 & TOI-4994 b & $1.103_{-0.033}^{+0.033}$ & $0.70_{-0.10}^{+0.10}$ & $1.19_{-0.50}^{+0.48}$ & $0.0753_{-0.0032}^{+0.0039}$ & $9.11_{-0.54}^{+0.46}$ & $0.50_{-0.32}^{+0.21}$ & $21.492045_{-0.000067}^{+0.000067}$ & $2363.6969_{-0.0014}^{+0.0014}$ & $0.22_{-0.22}^{+0.20}$ & $-10_{-0}^{+180}$ \\
280206394 & 677.01 & TOI-677 b & $1.303_{-0.037}^{+0.037}$ & $0.487_{-0.066}^{+0.066}$ & $2.16_{-0.13}^{+0.15}$ & $0.0895_{-0.0010}^{+0.0010}$ & $12.71_{-0.40}^{+0.39}$ & $0.726_{-0.019}^{+0.015}$ & $11.2365960_{-0.0000030}^{+0.0000030}$ & $3030.70523_{-0.00019}^{+0.00019}$ & $0.48_{-0.06}^{+0.18}$ & $150_{-120}^{+10}$ \\
286916251 & 1794.01 & TOI-1794 b & $1.323_{-0.029}^{+0.029}$ & $0.414_{-0.051}^{+0.051}$ & $0.62_{-0.38}^{+0.25}$ & $0.0244_{-0.0011}^{+0.0015}$ & $3.56_{-0.22}^{+0.19}$ & $0.46_{-0.31}^{+0.30}$ & $8.765509_{-0.000055}^{+0.000055}$ & $2661.9891_{-0.0044}^{+0.0044}$ & $0.12_{-0.12}^{+0.27}$ & $-170_{-160}^{+350}$ \\
287080092 & 1751.01 & TOI-1751 b & $1.322_{-0.030}^{+0.030}$ & $0.426_{-0.077}^{+0.077}$ & $0.38_{-0.20}^{+0.15}$ & $0.0212_{-0.0007}^{+0.0012}$ & $3.11_{-0.14}^{+0.16}$ & $0.48_{-0.32}^{+0.26}$ & $37.46855_{-0.00013}^{+0.00013}$ & $3532.1259_{-0.0042}^{+0.0042}$ & $0.02_{-0.02}^{+0.31}$ & $-150_{-30}^{+150}$ \\
287156968 & 1230.01 &  & $1.183_{-0.026}^{+0.026}$ & $0.599_{-0.082}^{+0.082}$ & $0.29_{-0.23}^{+0.23}$ & $0.0229_{-0.0018}^{+0.0041}$ & $3.15_{-0.45}^{+0.32}$ & $0.59_{-0.39}^{+0.30}$ & $25.05734_{-0.00017}^{+0.00017}$ & $1620.3121_{-0.0054}^{+0.0054}$ & $0.14_{-0.14}^{+0.31}$ & $-40_{-120}^{+20}$ \\
287256467 & 2141.01 & TOI-2141 b & $0.948_{-0.020}^{+0.020}$ & $1.19_{-0.12}^{+0.12}$ & $1.3_{-1.1}^{+1.1}$ & $0.0308_{-0.0015}^{+0.0031}$ & $3.28_{-0.28}^{+0.21}$ & $0.59_{-0.40}^{+0.30}$ & $18.261611_{-0.000095}^{+0.000095}$ & $3453.4310_{-0.0057}^{+0.0057}$ & $0.03_{-0.03}^{+0.36}$ & $-30_{-150}^{+60}$ \\
288132261 & 1258.01 &  & $1.507_{-0.030}^{+0.030}$ & $0.344_{-0.065}^{+0.065}$ & $0.38_{-0.15}^{+0.09}$ & $0.02773_{-0.00049}^{+0.00062}$ & $4.57_{-0.13}^{+0.12}$ & $0.38_{-0.25}^{+0.24}$ & $10.261298_{-0.000020}^{+0.000020}$ & $3333.6447_{-0.0021}^{+0.0021}$ & $0.03_{-0.03}^{+0.27}$ & $-20_{-160}^{+50}$ \\
288636599 & 1890.01 &  & $1.297_{-0.035}^{+0.035}$ & $0.466_{-0.069}^{+0.069}$ & $0.499_{-0.086}^{+0.078}$ & $0.07449_{-0.00085}^{+0.00092}$ & $10.56_{-0.30}^{+0.30}$ & $0.34_{-0.19}^{+0.13}$ & $19.967734_{-0.000026}^{+0.000026}$ & $2884.07232_{-0.00091}^{+0.00091}$ & $0.01_{-0.01}^{+0.23}$ & $-10_{-170}^{+50}$ \\
290403522 & 6798.01 &  & $1.491_{-0.041}^{+0.041}$ & $0.437_{-0.039}^{+0.039}$ & $0.073_{-0.013}^{+0.016}$ & $0.0778_{-0.0018}^{+0.0014}$ & $12.62_{-0.39}^{+0.46}$ & $0.43_{-0.22}^{+0.12}$ & $22.375244_{-0.000043}^{+0.000043}$ & $3136.5832_{-0.0026}^{+0.0026}$ & $0.57_{-0.09}^{+0.14}$ & $-122_{-13}^{+68}$ \\
294395926 & 678.01 &  & $1.029_{-0.024}^{+0.024}$ & $0.88_{-0.10}^{+0.10}$ & $0.67_{-0.40}^{+0.28}$ & $0.0286_{-0.0014}^{+0.0019}$ & $3.24_{-0.21}^{+0.19}$ & $0.48_{-0.32}^{+0.29}$ & $11.329872_{-0.000048}^{+0.000048}$ & $1493.0234_{-0.0033}^{+0.0033}$ & $0.02_{-0.02}^{+0.32}$ & $-30_{-140}^{+20}$ \\
294781547 & 1218.01 &  & $0.851_{-0.023}^{+0.023}$ & $1.50_{-0.17}^{+0.17}$ & $2.2_{-1.4}^{+1.0}$ & $0.0175_{-0.0011}^{+0.0012}$ & $1.64_{-0.12}^{+0.10}$ & $0.47_{-0.32}^{+0.31}$ & $13.773838_{-0.000066}^{+0.000066}$ & $1336.6318_{-0.0048}^{+0.0048}$ & $0.04_{-0.04}^{+0.34}$ & $180_{-200}^{+0}$ \\
299158887 & 1554.01 & Kepler-63 b & $0.905_{-0.028}^{+0.028}$ & $1.31_{-0.17}^{+0.17}$ & $2.5_{-1.2}^{+0.8}$ & $0.0590_{-0.0023}^{+0.0025}$ & $5.84_{-0.31}^{+0.29}$ & $0.43_{-0.29}^{+0.25}$ & $9.434157_{-0.000044}^{+0.000044}$ & $2444.8961_{-0.0012}^{+0.0012}$ & $0.32_{-0.26}^{+0.17}$ & $20_{-20}^{+150}$ \\
300038935 & 1228.01 & HD 56414 b & $1.870_{-0.065}^{+0.065}$ & $0.273_{-0.040}^{+0.040}$ & $0.34_{-0.15}^{+0.07}$ & $0.01995_{-0.00044}^{+0.00064}$ & $4.10_{-0.18}^{+0.17}$ & $0.36_{-0.24}^{+0.28}$ & $29.049690_{-0.000053}^{+0.000053}$ & $3178.4602_{-0.0018}^{+0.0018}$ & $0.01_{-0.01}^{+0.30}$ & $-170_{-140}^{+350}$ \\
300579472 & 4186.01 &  & $0.864_{-0.022}^{+0.022}$ & $1.38_{-0.14}^{+0.14}$ & $1.01_{-0.74}^{+0.57}$ & $0.0241_{-0.0018}^{+0.0029}$ & $2.34_{-0.24}^{+0.22}$ & $0.51_{-0.35}^{+0.33}$ & $12.750345_{-0.000057}^{+0.000057}$ & $3168.3384_{-0.0067}^{+0.0067}$ & $0.00_{-0.00}^{+0.37}$ & $-150_{-20}^{+140}$ \\
302773669 & 1573.01 & HD 17156 b & $1.522_{-0.039}^{+0.039}$ & $0.408_{-0.042}^{+0.042}$ & $3.46_{-0.28}^{+0.33}$ & $0.07474_{-0.00073}^{+0.00067}$ & $12.42_{-0.36}^{+0.32}$ & $0.509_{-0.054}^{+0.041}$ & $21.2164340_{-0.0000050}^{+0.0000050}$ & $3463.95302_{-0.00027}^{+0.00027}$ & $0.62_{-0.04}^{+0.14}$ & $67_{-39}^{+82}$ \\
303432813 & 5076.01 & TOI-5076 b & $0.807_{-0.019}^{+0.019}$ & $1.58_{-0.15}^{+0.15}$ & $0.79_{-0.46}^{+0.31}$ & $0.0407_{-0.0024}^{+0.0047}$ & $3.71_{-0.36}^{+0.28}$ & $0.42_{-0.29}^{+0.33}$ & $23.44327_{-0.00056}^{+0.00056}$ & $3250.889_{-0.018}^{+0.018}$ & $0.35_{-0.34}^{+0.09}$ & $-40_{-100}^{+10}$ \\
306249066 & 6596.01 &  & $1.132_{-0.027}^{+0.027}$ & $0.756_{-0.096}^{+0.096}$ & $0.67_{-0.11}^{+0.17}$ & $0.0857_{-0.0036}^{+0.0042}$ & $10.64_{-0.59}^{+0.49}$ & $0.875_{-0.033}^{+0.022}$ & $26.162179_{-0.000049}^{+0.000049}$ & $3059.0584_{-0.0014}^{+0.0014}$ & $0.00_{-0.00}^{+0.38}$ & $-160_{-20}^{+170}$ \\
308073360 & 3837.01 &  & $1.256_{-0.034}^{+0.034}$ & $0.468_{-0.061}^{+0.061}$ & $0.29_{-0.06}^{+0.12}$ & $0.0850_{-0.0029}^{+0.0019}$ & $11.54_{-0.45}^{+0.44}$ & $0.71_{-0.11}^{+0.05}$ & $11.888667_{-0.000031}^{+0.000031}$ & $2613.3812_{-0.0011}^{+0.0011}$ & $0.08_{-0.08}^{+0.30}$ & $-140_{-10}^{+120}$ \\
308098254 & 1906.01 & WASP-162 b & $1.193_{-0.036}^{+0.036}$ & $0.563_{-0.067}^{+0.067}$ & $0.83_{-0.16}^{+0.08}$ & $0.0898_{-0.0015}^{+0.0020}$ & $11.74_{-0.41}^{+0.42}$ & $0.25_{-0.17}^{+0.20}$ & $9.624676_{-0.000010}^{+0.000010}$ & $2299.07665_{-0.00058}^{+0.00058}$ & $0.14_{-0.08}^{+0.27}$ & $10_{-0}^{+170}$ \\
309791156 & 533.01 &  & $0.788_{-0.020}^{+0.020}$ & $1.74_{-0.16}^{+0.16}$ & $1.31_{-0.61}^{+0.46}$ & $0.0394_{-0.0011}^{+0.0018}$ & $3.43_{-0.16}^{+0.15}$ & $0.46_{-0.31}^{+0.24}$ & $19.571591_{-0.000023}^{+0.000023}$ & $1332.6969_{-0.0014}^{+0.0014}$ & $0.03_{-0.03}^{+0.29}$ & $-150_{-20}^{+130}$ \\
313194972 & 4144.01 &  & $0.893_{-0.022}^{+0.022}$ & $1.31_{-0.13}^{+0.13}$ & $0.641_{-0.092}^{+0.054}$ & $0.1115_{-0.0017}^{+0.0021}$ & $10.89_{-0.33}^{+0.33}$ & $0.25_{-0.17}^{+0.16}$ & $16.902051_{-0.000020}^{+0.000020}$ & $2744.99054_{-0.00055}^{+0.00055}$ & $0.26_{-0.08}^{+0.24}$ & $-140_{-6}^{+87}$ \\
314865962 & 208.01 &  & $0.975_{-0.025}^{+0.025}$ & $1.05_{-0.11}^{+0.11}$ & $0.47_{-0.34}^{+0.29}$ & $0.0270_{-0.0019}^{+0.0029}$ & $2.94_{-0.30}^{+0.23}$ & $0.52_{-0.35}^{+0.32}$ & $22.4540_{-0.0028}^{+0.0028}$ & $1335.9696_{-0.0098}^{+0.0098}$ & $0.17_{-0.17}^{+0.29}$ & $-140_{-10}^{+110}$ \\
316468545 & 2050.01 &  & $0.887_{-0.020}^{+0.020}$ & $1.39_{-0.13}^{+0.13}$ & $1.8_{-1.7}^{+1.4}$ & $0.0224_{-0.0021}^{+0.0067}$ & $2.46_{-0.48}^{+0.38}$ & $0.56_{-0.38}^{+0.37}$ & $13.597033_{-0.000093}^{+0.000093}$ & $3427.4342_{-0.0074}^{+0.0074}$ & $0.03_{-0.03}^{+0.39}$ & $-160_{-110}^{+340}$ \\
318753380 & 2443.01 & TOI-2443 b & $0.666_{-0.027}^{+0.027}$ & $2.26_{-0.31}^{+0.31}$ & $0.57_{-0.41}^{+0.37}$ & $0.0350_{-0.0028}^{+0.0043}$ & $2.61_{-0.29}^{+0.26}$ & $0.50_{-0.34}^{+0.33}$ & $15.6694_{-0.0089}^{+0.0089}$ & $2148.1001_{-0.0061}^{+0.0061}$ & $0.48_{-0.25}^{+0.24}$ & $-52_{-78}^{+5}$ \\
320004517 & 1055.01 & HD 183579 b & $0.971_{-0.021}^{+0.021}$ & $1.14_{-0.17}^{+0.17}$ & $1.13_{-0.44}^{+0.25}$ & $0.03220_{-0.00074}^{+0.00098}$ & $3.43_{-0.12}^{+0.10}$ & $0.38_{-0.25}^{+0.25}$ & $17.471315_{-0.000021}^{+0.000021}$ & $1661.0629_{-0.0015}^{+0.0015}$ & $0.02_{-0.02}^{+0.27}$ & $-160_{-20}^{+170}$ \\
322807675 & 2398.01 &  & $0.853_{-0.021}^{+0.021}$ & $1.42_{-0.14}^{+0.14}$ & $3.4_{-0.7}^{+3.4}$ & $0.108_{-0.011}^{+0.005}$ & $9.68_{-0.70}^{+0.85}$ & $0.82_{-0.22}^{+0.04}$ & $19.406095_{-0.000024}^{+0.000024}$ & $2285.44025_{-0.00066}^{+0.00066}$ & $0.01_{-0.01}^{+0.51}$ & $0_{-10}^{+170}$ \\
327301957 & 1074.01 &  & $0.745_{-0.019}^{+0.019}$ & $1.94_{-0.20}^{+0.20}$ & $1.27_{-0.76}^{+0.51}$ & $0.0333_{-0.0020}^{+0.0027}$ & $2.75_{-0.20}^{+0.21}$ & $0.46_{-0.31}^{+0.30}$ & $13.942929_{-0.000058}^{+0.000058}$ & $1662.6493_{-0.0036}^{+0.0036}$ & $0.11_{-0.11}^{+0.26}$ & $-40_{-120}^{+20}$ \\
327579226 & 1532.01 &  & $1.430_{-0.034}^{+0.034}$ & $0.460_{-0.054}^{+0.054}$ & $1.00_{-0.33}^{+0.75}$ & $0.0784_{-0.0053}^{+0.0034}$ & $12.03_{-0.77}^{+0.72}$ & $0.76_{-0.16}^{+0.07}$ & $8.905399_{-0.000012}^{+0.000012}$ & $3446.0010_{-0.0015}^{+0.0015}$ & $0.33_{-0.32}^{+0.17}$ & $170_{-170}^{+10}$ \\
327917279 & 6819.01 &  & $1.460_{-0.035}^{+0.035}$ & $0.325_{-0.054}^{+0.054}$ & $0.26_{-0.22}^{+0.34}$ & $0.047_{-0.006}^{+0.019}$ & $8.8_{-2.2}^{+1.7}$ & $0.68_{-0.46}^{+0.27}$ & $8.546727_{-0.000059}^{+0.000059}$ & $3168.7739_{-0.0038}^{+0.0038}$ & $0.05_{-0.05}^{+0.39}$ & $-150_{-30}^{+170}$ \\
328012209 & 2309.01 &  & $1.323_{-0.026}^{+0.026}$ & $0.489_{-0.070}^{+0.070}$ & $0.33_{-0.22}^{+0.15}$ & $0.0277_{-0.0014}^{+0.0023}$ & $4.09_{-0.30}^{+0.24}$ & $0.48_{-0.33}^{+0.32}$ & $20.26562_{-0.00013}^{+0.00013}$ & $2044.3332_{-0.0045}^{+0.0045}$ & $0.03_{-0.03}^{+0.34}$ & $-150_{-20}^{+130}$ \\
328502522 & 6457.01 &  & $1.405_{-0.034}^{+0.034}$ & $0.484_{-0.089}^{+0.089}$ & $0.29_{-0.22}^{+0.20}$ & $0.068_{-0.006}^{+0.012}$ & $11.0_{-1.5}^{+1.2}$ & $0.52_{-0.35}^{+0.34}$ & $41.41848_{-0.00073}^{+0.00073}$ & $3280.042_{-0.010}^{+0.010}$ & $0.03_{-0.03}^{+0.38}$ & $-130_{-30}^{+120}$ \\
328934463 & 2485.01 & TOI-2485 b & $1.790_{-0.047}^{+0.047}$ & $0.203_{-0.031}^{+0.031}$ & $0.11_{-0.04}^{+0.12}$ & $0.0725_{-0.0036}^{+0.0031}$ & $14.10_{-0.73}^{+0.73}$ & $0.70_{-0.33}^{+0.10}$ & $11.23481_{-0.00027}^{+0.00027}$ & $2658.812_{-0.017}^{+0.017}$ & $0.12_{-0.12}^{+0.30}$ & $-40_{-130}^{+20}$ \\
330690135 & 5170.01 & K2-333 b & $1.208_{-0.030}^{+0.030}$ & $0.67_{-0.13}^{+0.13}$ & $0.65_{-0.29}^{+0.17}$ & $0.0449_{-0.0019}^{+0.0020}$ & $5.94_{-0.31}^{+0.29}$ & $0.38_{-0.26}^{+0.27}$ & $14.7571_{-0.0017}^{+0.0017}$ & $2558.6194_{-0.0028}^{+0.0028}$ & $0.00_{-0.00}^{+0.30}$ & $-20_{-160}^{+40}$ \\
332564140 & 5400.01 &  & $0.947_{-0.028}^{+0.028}$ & $1.03_{-0.15}^{+0.15}$ & $0.93_{-0.56}^{+0.39}$ & $0.0447_{-0.0022}^{+0.0034}$ & $4.69_{-0.35}^{+0.28}$ & $0.47_{-0.32}^{+0.30}$ & $19.806653_{-0.000075}^{+0.000075}$ & $2970.5295_{-0.0032}^{+0.0032}$ & $0.00_{-0.00}^{+0.33}$ & $-30_{-150}^{+30}$ \\
332660150 & 938.01 &  & $0.993_{-0.025}^{+0.025}$ & $1.08_{-0.14}^{+0.14}$ & $0.36_{-0.24}^{+0.22}$ & $0.0450_{-0.0031}^{+0.0043}$ & $4.96_{-0.43}^{+0.41}$ & $0.52_{-0.35}^{+0.29}$ & $8.80737_{-0.00016}^{+0.00016}$ & $2193.805_{-0.013}^{+0.013}$ & $0.36_{-0.20}^{+0.28}$ & $-48_{-88}^{+8}$ \\
334305570 & 777.01 &  & $1.525_{-0.038}^{+0.038}$ & $0.405_{-0.042}^{+0.042}$ & $0.41_{-0.11}^{+0.08}$ & $0.0477_{-0.0008}^{+0.0010}$ & $7.96_{-0.25}^{+0.25}$ & $0.37_{-0.24}^{+0.18}$ & $8.300855_{-0.000010}^{+0.000010}$ & $1575.7807_{-0.0016}^{+0.0016}$ & $0.01_{-0.01}^{+0.24}$ & $-160_{-20}^{+180}$ \\
335655755 & 4132.01 &  & $1.804_{-0.044}^{+0.044}$ & $0.195_{-0.023}^{+0.023}$ & $0.64_{-0.20}^{+0.24}$ & $0.0643_{-0.0018}^{+0.0020}$ & $12.69_{-0.45}^{+0.52}$ & $0.48_{-0.28}^{+0.16}$ & $11.764776_{-0.000022}^{+0.000022}$ & $2395.93758_{-0.00069}^{+0.00069}$ & $0.41_{-0.11}^{+0.24}$ & $130_{-120}^{+10}$ \\
336126253 & 5193.01 &  & $0.885_{-0.022}^{+0.022}$ & $1.35_{-0.14}^{+0.14}$ & $1.42_{-0.72}^{+0.54}$ & $0.0587_{-0.0029}^{+0.0030}$ & $5.68_{-0.30}^{+0.33}$ & $0.44_{-0.29}^{+0.27}$ & $18.99711_{-0.00011}^{+0.00011}$ & $2408.1531_{-0.0027}^{+0.0027}$ & $0.01_{-0.01}^{+0.31}$ & $-160_{-20}^{+180}$ \\
339207847 & 3727.01 &  & $1.482_{-0.042}^{+0.042}$ & $0.423_{-0.064}^{+0.064}$ & $0.88_{-0.38}^{+0.30}$ & $0.0760_{-0.0036}^{+0.0054}$ & $12.46_{-0.78}^{+0.80}$ & $0.45_{-0.30}^{+0.24}$ & $13.41131_{-0.00062}^{+0.00062}$ & $2919.6318_{-0.0015}^{+0.0015}$ & $0.32_{-0.21}^{+0.23}$ & $170_{-170}^{+10}$ \\
339672028 & 481.01 & TOI-481 b & $1.698_{-0.038}^{+0.038}$ & $0.251_{-0.045}^{+0.045}$ & $0.386_{-0.028}^{+0.016}$ & $0.06169_{-0.00025}^{+0.00036}$ & $11.44_{-0.24}^{+0.28}$ & $0.18_{-0.12}^{+0.10}$ & $10.3311560_{-0.0000020}^{+0.0000020}$ & $3205.95134_{-0.00021}^{+0.00021}$ & $0.20_{-0.14}^{+0.21}$ & $10_{-0}^{+160}$ \\
341630071 & 2147.01 &  & $1.393_{-0.030}^{+0.030}$ & $0.386_{-0.065}^{+0.065}$ & $0.87_{-0.16}^{+0.07}$ & $0.0706_{-0.0010}^{+0.0010}$ & $10.74_{-0.30}^{+0.25}$ & $0.22_{-0.15}^{+0.19}$ & $26.205158_{-0.000048}^{+0.000048}$ & $2599.17708_{-0.00082}^{+0.00082}$ & $0.31_{-0.11}^{+0.23}$ & $150_{-130}^{+20}$ \\
341815197 & 2089.01 &  & $0.815_{-0.018}^{+0.018}$ & $1.63_{-0.18}^{+0.18}$ & $1.24_{-0.89}^{+0.78}$ & $0.0371_{-0.0023}^{+0.0037}$ & $3.38_{-0.28}^{+0.26}$ & $0.54_{-0.36}^{+0.30}$ & $49.99499_{-0.00045}^{+0.00045}$ & $2790.2834_{-0.0055}^{+0.0055}$ & $0.05_{-0.05}^{+0.32}$ & $-150_{-30}^{+140}$ \\
342642208 & 2158.01 & TOI-2158 b & $1.430_{-0.037}^{+0.037}$ & $0.363_{-0.055}^{+0.055}$ & $0.74_{-0.40}^{+0.56}$ & $0.0651_{-0.0051}^{+0.0066}$ & $10.31_{-0.91}^{+0.95}$ & $0.60_{-0.38}^{+0.19}$ & $8.600753_{-0.000048}^{+0.000048}$ & $2758.5862_{-0.0019}^{+0.0019}$ & $0.30_{-0.26}^{+0.20}$ & $10_{-10}^{+160}$ \\
343019899 & 1386.01 & TOI-1386 c & $1.009_{-0.024}^{+0.024}$ & $1.01_{-0.11}^{+0.11}$ & $0.73_{-0.38}^{+0.28}$ & $0.0494_{-0.0021}^{+0.0023}$ & $5.45_{-0.28}^{+0.27}$ & $0.46_{-0.31}^{+0.27}$ & $25.83862_{-0.00015}^{+0.00015}$ & $3561.0175_{-0.0063}^{+0.0063}$ & $0.00_{-0.00}^{+0.34}$ & $-40_{-130}^{+20}$ \\
346929661 & 2043.01 &  & $1.222_{-0.027}^{+0.027}$ & $0.575_{-0.080}^{+0.080}$ & $0.36_{-0.32}^{+0.38}$ & $0.0341_{-0.0039}^{+0.0098}$ & $5.0_{-1.0}^{+0.8}$ & $0.59_{-0.40}^{+0.34}$ & $12.01352_{-0.00018}^{+0.00018}$ & $3428.027_{-0.020}^{+0.020}$ & $0.05_{-0.05}^{+0.39}$ & $-30_{-150}^{+30}$ \\
347357977 & 2370.01 &  & $1.050_{-0.023}^{+0.023}$ & $0.96_{-0.11}^{+0.11}$ & $0.86_{-0.51}^{+0.36}$ & $0.0490_{-0.0026}^{+0.0036}$ & $5.68_{-0.44}^{+0.30}$ & $0.47_{-0.32}^{+0.29}$ & $12.682594_{-0.000084}^{+0.000084}$ & $2262.5114_{-0.0027}^{+0.0027}$ & $0.01_{-0.01}^{+0.32}$ & $-30_{-150}^{+30}$ \\
350020859 & 5141.01 & HD 89345 b & $1.788_{-0.041}^{+0.041}$ & $0.201_{-0.027}^{+0.027}$ & $0.41_{-0.13}^{+0.05}$ & $0.03639_{-0.00077}^{+0.00088}$ & $7.10_{-0.25}^{+0.20}$ & $0.29_{-0.20}^{+0.25}$ & $11.8148_{-0.0010}^{+0.0010}$ & $2556.00478_{-0.00098}^{+0.00098}$ & $0.30_{-0.16}^{+0.21}$ & $10_{-10}^{+140}$ \\
353782445 & 1664.01 &  & $1.336_{-0.031}^{+0.031}$ & $0.480_{-0.064}^{+0.064}$ & $4.1_{-2.6}^{+1.9}$ & $0.0172_{-0.0008}^{+0.0011}$ & $2.53_{-0.16}^{+0.14}$ & $0.50_{-0.34}^{+0.29}$ & $11.835088_{-0.000027}^{+0.000027}$ & $3559.1379_{-0.0028}^{+0.0028}$ & $0.67_{-0.12}^{+0.16}$ & $88_{-64}^{+59}$ \\
355895977 & 6661.01 &  & $0.775_{-0.018}^{+0.018}$ & $1.81_{-0.17}^{+0.17}$ & $1.21_{-0.90}^{+0.84}$ & $0.0371_{-0.0027}^{+0.0045}$ & $3.23_{-0.33}^{+0.29}$ & $0.55_{-0.37}^{+0.31}$ & $10.578863_{-0.000095}^{+0.000095}$ & $2425.1999_{-0.0036}^{+0.0036}$ & $0.00_{-0.00}^{+0.39}$ & $-140_{-30}^{+130}$ \\
356311210 & 1261.01 &  & $1.125_{-0.034}^{+0.034}$ & $0.638_{-0.090}^{+0.090}$ & $1.9_{-1.2}^{+0.9}$ & $0.0320_{-0.0016}^{+0.0021}$ & $3.97_{-0.27}^{+0.23}$ & $0.49_{-0.33}^{+0.28}$ & $18.05743_{-0.00011}^{+0.00011}$ & $2628.7681_{-0.0018}^{+0.0018}$ & $0.42_{-0.21}^{+0.23}$ & $30_{-10}^{+140}$ \\
356472238 & 5382.01 &  & $1.752_{-0.038}^{+0.038}$ & $0.239_{-0.032}^{+0.032}$ & $0.50_{-0.34}^{+0.24}$ & $0.0258_{-0.0017}^{+0.0032}$ & $5.12_{-0.57}^{+0.39}$ & $0.50_{-0.33}^{+0.32}$ & $14.54158_{-0.00031}^{+0.00031}$ & $2961.9385_{-0.0052}^{+0.0052}$ & $0.36_{-0.35}^{+0.12}$ & $160_{-160}^{+20}$ \\
358248442 & 2419.01 &  & $1.397_{-0.047}^{+0.047}$ & $0.364_{-0.061}^{+0.061}$ & $0.30_{-0.15}^{+0.12}$ & $0.0325_{-0.0011}^{+0.0012}$ & $4.96_{-0.24}^{+0.25}$ & $0.48_{-0.31}^{+0.25}$ & $18.881109_{-0.000056}^{+0.000056}$ & $3169.7760_{-0.0035}^{+0.0035}$ & $0.09_{-0.09}^{+0.24}$ & $-20_{-150}^{+20}$ \\
358460246 & 867.01 &  & $1.164_{-0.028}^{+0.028}$ & $0.650_{-0.090}^{+0.090}$ & $0.63_{-0.44}^{+0.32}$ & $0.0174_{-0.0010}^{+0.0016}$ & $2.26_{-0.18}^{+0.17}$ & $0.49_{-0.33}^{+0.32}$ & $15.404357_{-0.000072}^{+0.000072}$ & $1326.1830_{-0.0047}^{+0.0047}$ & $0.02_{-0.02}^{+0.33}$ & $-20_{-160}^{+40}$ \\
360714300 & 3359.01 &  & $0.989_{-0.022}^{+0.022}$ & $1.05_{-0.13}^{+0.13}$ & $0.75_{-0.46}^{+0.30}$ & $0.0239_{-0.0011}^{+0.0012}$ & $2.59_{-0.14}^{+0.13}$ & $0.46_{-0.31}^{+0.31}$ & $15.811901_{-0.000078}^{+0.000078}$ & $3014.0001_{-0.0034}^{+0.0034}$ & $0.00_{-0.00}^{+0.35}$ & $-150_{-20}^{+130}$ \\
363914762 & 812.01 &  & $1.628_{-0.041}^{+0.041}$ & $0.301_{-0.033}^{+0.033}$ & $0.317_{-0.053}^{+0.048}$ & $0.07789_{-0.00091}^{+0.00089}$ & $13.84_{-0.40}^{+0.37}$ & $0.34_{-0.20}^{+0.13}$ & $13.866600_{-0.000021}^{+0.000021}$ & $2249.58818_{-0.00084}^{+0.00084}$ & $0.02_{-0.02}^{+0.21}$ & $-20_{-160}^{+50}$ \\
364395234 & 1232.01 &  & $1.114_{-0.031}^{+0.031}$ & $0.70_{-0.11}^{+0.11}$ & $0.197_{-0.021}^{+0.025}$ & $0.0907_{-0.0018}^{+0.0024}$ & $11.07_{-0.41}^{+0.39}$ & $0.854_{-0.020}^{+0.017}$ & $14.254487_{-0.000019}^{+0.000019}$ & $1544.0282_{-0.0012}^{+0.0012}$ & $0.45_{-0.10}^{+0.19}$ & $-129_{-6}^{+63}$ \\
365673804 & 1735.01 &  & $1.290_{-0.030}^{+0.030}$ & $0.569_{-0.054}^{+0.054}$ & $1.17_{-0.84}^{+0.61}$ & $0.0178_{-0.0008}^{+0.0013}$ & $2.55_{-0.17}^{+0.14}$ & $0.52_{-0.35}^{+0.32}$ & $10.385749_{-0.000026}^{+0.000026}$ & $3395.9430_{-0.0025}^{+0.0025}$ & $0.30_{-0.27}^{+0.20}$ & $10_{-10}^{+170}$ \\
366410512 & 5101.01 & K2-98 b & $1.575_{-0.045}^{+0.045}$ & $0.272_{-0.036}^{+0.036}$ & $0.23_{-0.20}^{+0.18}$ & $0.0310_{-0.0024}^{+0.0052}$ & $5.61_{-0.71}^{+0.62}$ & $0.55_{-0.38}^{+0.35}$ & $10.136693_{-0.000062}^{+0.000062}$ & $3247.8174_{-0.0087}^{+0.0087}$ & $0.02_{-0.02}^{+0.37}$ & $-160_{-20}^{+170}$ \\
366989877 & 1054.01 &  & $1.192_{-0.025}^{+0.025}$ & $0.60_{-0.10}^{+0.10}$ & $0.56_{-0.33}^{+0.20}$ & $0.0231_{-0.0010}^{+0.0013}$ & $3.03_{-0.17}^{+0.15}$ & $0.45_{-0.31}^{+0.30}$ & $15.50764_{-0.00022}^{+0.00022}$ & $3122.691_{-0.016}^{+0.016}$ & $0.01_{-0.01}^{+0.31}$ & $-150_{-30}^{+160}$ \\
371573539 & 6148.01 &  & $1.800_{-0.050}^{+0.050}$ & $0.201_{-0.023}^{+0.023}$ & $2.7_{-1.1}^{+0.6}$ & $0.0624_{-0.0026}^{+0.0026}$ & $12.22_{-0.60}^{+0.60}$ & $0.35_{-0.24}^{+0.27}$ & $8.3688_{-0.0019}^{+0.0019}$ & $2849.6237_{-0.0022}^{+0.0022}$ & $0.71_{-0.04}^{+0.13}$ & $110_{-73}^{+37}$ \\
373017346 & 4450.01 &  & $1.136_{-0.028}^{+0.028}$ & $0.690_{-0.095}^{+0.095}$ & $0.94_{-0.51}^{+0.44}$ & $0.0344_{-0.0014}^{+0.0020}$ & $4.33_{-0.23}^{+0.23}$ & $0.51_{-0.33}^{+0.24}$ & $10.692494_{-0.000030}^{+0.000030}$ & $2759.8775_{-0.0013}^{+0.0013}$ & $0.03_{-0.03}^{+0.33}$ & $-10_{-10}^{+190}$ \\
374997123 & 1222.01 &  & $1.337_{-0.029}^{+0.029}$ & $0.431_{-0.065}^{+0.065}$ & $4.8_{-3.4}^{+2.4}$ & $0.0173_{-0.0010}^{+0.0013}$ & $2.56_{-0.19}^{+0.16}$ & $0.50_{-0.33}^{+0.33}$ & $10.194439_{-0.000036}^{+0.000036}$ & $1329.4705_{-0.0037}^{+0.0037}$ & $0.74_{-0.11}^{+0.14}$ & $106_{-73}^{+48}$ \\
380671216 & 5495.01 &  & $1.015_{-0.028}^{+0.028}$ & $0.91_{-0.13}^{+0.13}$ & $0.26_{-0.22}^{+0.30}$ & $0.0286_{-0.0030}^{+0.0056}$ & $3.35_{-0.54}^{+0.42}$ & $0.54_{-0.37}^{+0.36}$ & $9.65685_{-0.00072}^{+0.00072}$ & $2559.900_{-0.012}^{+0.012}$ & $0.20_{-0.20}^{+0.33}$ & $-130_{-30}^{+100}$ \\
380836882 & 2526.01 &  & $1.325_{-0.029}^{+0.029}$ & $0.444_{-0.068}^{+0.068}$ & $0.439_{-0.079}^{+0.040}$ & $0.0827_{-0.0014}^{+0.0015}$ & $11.97_{-0.33}^{+0.33}$ & $0.24_{-0.16}^{+0.19}$ & $8.011402_{-0.000010}^{+0.000010}$ & $2381.86807_{-0.00068}^{+0.00068}$ & $0.00_{-0.00}^{+0.24}$ & $-20_{-160}^{+20}$ \\
382045742 & 3355.01 &  & $1.186_{-0.031}^{+0.031}$ & $0.601_{-0.089}^{+0.089}$ & $0.51_{-0.33}^{+0.23}$ & $0.0190_{-0.0012}^{+0.0015}$ & $2.49_{-0.19}^{+0.17}$ & $0.48_{-0.33}^{+0.31}$ & $15.660208_{-0.000084}^{+0.000084}$ & $2362.1513_{-0.0033}^{+0.0033}$ & $0.04_{-0.04}^{+0.30}$ & $-150_{-30}^{+150}$ \\
382626661 & 283.01 &  & $0.792_{-0.019}^{+0.019}$ & $1.72_{-0.17}^{+0.17}$ & $1.64_{-0.69}^{+0.36}$ & $0.02489_{-0.00062}^{+0.00080}$ & $2.160_{-0.085}^{+0.075}$ & $0.37_{-0.25}^{+0.26}$ & $17.617457_{-0.000020}^{+0.000020}$ & $3165.6929_{-0.0011}^{+0.0011}$ & $0.00_{-0.00}^{+0.28}$ & $-160_{-20}^{+160}$ \\
383721338 & 4553.01 &  & $1.476_{-0.031}^{+0.031}$ & $0.369_{-0.059}^{+0.059}$ & $0.359_{-0.046}^{+0.024}$ & $0.06700_{-0.00071}^{+0.00076}$ & $10.79_{-0.24}^{+0.26}$ & $0.21_{-0.14}^{+0.15}$ & $20.313826_{-0.000062}^{+0.000062}$ & $2422.81684_{-0.00081}^{+0.00081}$ & $0.00_{-0.00}^{+0.24}$ & $-20_{-160}^{+20}$ \\
390151888 & 6543.01 &  & $1.157_{-0.029}^{+0.029}$ & $0.66_{-0.11}^{+0.11}$ & $0.35_{-0.28}^{+0.23}$ & $0.0278_{-0.0021}^{+0.0053}$ & $3.77_{-0.49}^{+0.45}$ & $0.54_{-0.37}^{+0.33}$ & $15.55243_{-0.00010}^{+0.00010}$ & $3067.8516_{-0.0080}^{+0.0080}$ & $0.04_{-0.04}^{+0.38}$ & $-140_{-20}^{+120}$ \\
391904697 & 705.01 &  & $0.825_{-0.021}^{+0.021}$ & $1.53_{-0.16}^{+0.16}$ & $0.85_{-0.64}^{+0.61}$ & $0.0331_{-0.0025}^{+0.0039}$ & $3.07_{-0.30}^{+0.28}$ & $0.54_{-0.37}^{+0.31}$ & $47.01986_{-0.00050}^{+0.00050}$ & $1352.127_{-0.010}^{+0.010}$ & $0.00_{-0.00}^{+0.42}$ & $-140_{-20}^{+120}$ \\
394050135 & 2025.01 & TOI-2025 b & $1.525_{-0.034}^{+0.034}$ & $0.289_{-0.040}^{+0.040}$ & $0.85_{-0.12}^{+0.20}$ & $0.0759_{-0.0018}^{+0.0012}$ & $12.57_{-0.37}^{+0.38}$ & $0.53_{-0.13}^{+0.07}$ & $8.8720790_{-0.0000050}^{+0.0000050}$ & $2754.93956_{-0.00033}^{+0.00033}$ & $0.39_{-0.11}^{+0.21}$ & $30_{-10}^{+130}$ \\
394223845 & 4820.01 &  & $1.402_{-0.046}^{+0.046}$ & $0.396_{-0.062}^{+0.062}$ & $1.5_{-0.9}^{+1.3}$ & $0.0720_{-0.0048}^{+0.0055}$ & $11.09_{-0.88}^{+0.85}$ & $0.62_{-0.40}^{+0.19}$ & $27.13545_{-0.00012}^{+0.00012}$ & $2246.3998_{-0.0028}^{+0.0028}$ & $0.53_{-0.25}^{+0.23}$ & $130_{-120}^{+30}$ \\
394287035 & 2328.01 &  & $0.958_{-0.024}^{+0.024}$ & $0.98_{-0.11}^{+0.11}$ & $2.60_{-0.56}^{+0.59}$ & $0.0955_{-0.0024}^{+0.0020}$ & $9.96_{-0.31}^{+0.35}$ & $0.42_{-0.23}^{+0.14}$ & $17.101952_{-0.000014}^{+0.000014}$ & $2356.60779_{-0.00046}^{+0.00046}$ & $0.36_{-0.12}^{+0.20}$ & $130_{-110}^{+40}$ \\
399871011 & 943.01 &  & $1.490_{-0.034}^{+0.034}$ & $0.437_{-0.048}^{+0.048}$ & $0.32_{-0.12}^{+0.08}$ & $0.0821_{-0.0021}^{+0.0037}$ & $13.53_{-0.61}^{+0.51}$ & $0.41_{-0.27}^{+0.24}$ & $12.362623_{-0.000036}^{+0.000036}$ & $1444.2672_{-0.0014}^{+0.0014}$ & $0.06_{-0.06}^{+0.26}$ & $-30_{-130}^{+10}$ \\
405559035 & 2037.01 &  & $1.227_{-0.025}^{+0.025}$ & $0.599_{-0.079}^{+0.079}$ & $0.30_{-0.23}^{+0.22}$ & $0.0269_{-0.0020}^{+0.0036}$ & $3.73_{-0.44}^{+0.32}$ & $0.55_{-0.37}^{+0.31}$ & $11.15193_{-0.00016}^{+0.00016}$ & $2706.7296_{-0.0079}^{+0.0079}$ & $0.02_{-0.02}^{+0.42}$ & $-40_{-120}^{+20}$ \\
407126408 & 913.01 & TOI-913 b & $0.704_{-0.022}^{+0.022}$ & $2.10_{-0.24}^{+0.24}$ & $1.38_{-0.79}^{+0.55}$ & $0.0315_{-0.0014}^{+0.0018}$ & $2.44_{-0.14}^{+0.15}$ & $0.47_{-0.31}^{+0.28}$ & $11.099348_{-0.000022}^{+0.000022}$ & $1625.2127_{-0.0024}^{+0.0024}$ & $0.00_{-0.00}^{+0.36}$ & $-140_{-20}^{+120}$ \\
407905370 & 3573.01 &  & $1.489_{-0.038}^{+0.038}$ & $0.352_{-0.059}^{+0.059}$ & $1.4_{-1.0}^{+0.8}$ & $0.074_{-0.006}^{+0.011}$ & $12.6_{-1.5}^{+1.2}$ & $0.49_{-0.33}^{+0.35}$ & $9.8128_{-0.0024}^{+0.0024}$ & $1747.7941_{-0.0034}^{+0.0034}$ & $0.53_{-0.23}^{+0.20}$ & $120_{-100}^{+40}$ \\
408114363 & 2450.01 &  & $0.789_{-0.021}^{+0.021}$ & $1.75_{-0.19}^{+0.19}$ & $1.25_{-0.50}^{+0.34}$ & $0.0760_{-0.0032}^{+0.0037}$ & $6.57_{-0.38}^{+0.31}$ & $0.38_{-0.26}^{+0.25}$ & $17.88520_{-0.00011}^{+0.00011}$ & $2179.1757_{-0.0024}^{+0.0024}$ & $0.09_{-0.09}^{+0.25}$ & $-150_{-10}^{+130}$ \\
408137826 & 941.01 &  & $1.195_{-0.040}^{+0.040}$ & $0.62_{-0.10}^{+0.10}$ & $0.74_{-0.30}^{+0.18}$ & $0.0534_{-0.0017}^{+0.0018}$ & $6.97_{-0.33}^{+0.32}$ & $0.39_{-0.26}^{+0.26}$ & $8.514599_{-0.000039}^{+0.000039}$ & $2198.2769_{-0.0014}^{+0.0014}$ & $0.04_{-0.04}^{+0.27}$ & $-20_{-10}^{+200}$ \\
408508003 & 6862.01 &  & $1.263_{-0.035}^{+0.035}$ & $0.501_{-0.072}^{+0.072}$ & $0.88_{-0.35}^{+0.29}$ & $0.0918_{-0.0034}^{+0.0041}$ & $12.71_{-0.63}^{+0.60}$ & $0.44_{-0.29}^{+0.21}$ & $8.224205_{-0.000089}^{+0.000089}$ & $3225.5472_{-0.0081}^{+0.0081}$ & $0.19_{-0.18}^{+0.24}$ & $10_{-20}^{+150}$ \\
409794137 & 1478.01 & TOI-1478 b & $1.030_{-0.024}^{+0.024}$ & $0.83_{-0.10}^{+0.10}$ & $0.96_{-0.13}^{+0.17}$ & $0.0939_{-0.0019}^{+0.0018}$ & $10.55_{-0.31}^{+0.35}$ & $0.42_{-0.15}^{+0.09}$ & $10.1802210_{-0.0000050}^{+0.0000050}$ & $2982.23815_{-0.00042}^{+0.00042}$ & $0.01_{-0.01}^{+0.25}$ & $-170_{-150}^{+350}$ \\
410214986 & 200.01 & DS Tuc A b & $0.955_{-0.031}^{+0.031}$ & $1.05_{-0.15}^{+0.15}$ & $1.41_{-0.16}^{+0.20}$ & $0.04824_{-0.00075}^{+0.00075}$ & $5.02_{-0.18}^{+0.17}$ & $0.39_{-0.12}^{+0.08}$ & $8.1382210_{-0.0000020}^{+0.0000020}$ & $1332.30839_{-0.00030}^{+0.00030}$ & $0.12_{-0.12}^{+0.21}$ & $-170_{-170}^{+350}$ \\
417931607 & 1451.01 & TOI-1451 b & $1.035_{-0.022}^{+0.022}$ & $0.80_{-0.11}^{+0.11}$ & $2.6_{-1.7}^{+1.1}$ & $0.0233_{-0.0013}^{+0.0022}$ & $2.70_{-0.22}^{+0.19}$ & $0.48_{-0.32}^{+0.31}$ & $16.537892_{-0.000090}^{+0.000090}$ & $3348.1018_{-0.0066}^{+0.0066}$ & $0.47_{-0.21}^{+0.22}$ & $40_{-30}^{+120}$ \\
424391516 & 1761.01 &  & $1.213_{-0.026}^{+0.026}$ & $0.653_{-0.079}^{+0.079}$ & $0.80_{-0.62}^{+0.48}$ & $0.0191_{-0.0013}^{+0.0027}$ & $2.64_{-0.30}^{+0.24}$ & $0.52_{-0.35}^{+0.34}$ & $11.592218_{-0.000081}^{+0.000081}$ & $2714.9172_{-0.0039}^{+0.0039}$ & $0.03_{-0.03}^{+0.34}$ & $-170_{-120}^{+350}$ \\
432280671 & 6012.01 &  & $1.208_{-0.027}^{+0.027}$ & $0.564_{-0.092}^{+0.092}$ & $0.48_{-0.27}^{+0.21}$ & $0.0575_{-0.0033}^{+0.0039}$ & $7.63_{-0.51}^{+0.50}$ & $0.46_{-0.31}^{+0.28}$ & $16.2099_{-0.0078}^{+0.0078}$ & $2861.6596_{-0.0054}^{+0.0054}$ & $0.05_{-0.05}^{+0.28}$ & $-30_{-150}^{+30}$ \\
437756191 & 6203.01 &  & $1.330_{-0.031}^{+0.031}$ & $0.442_{-0.062}^{+0.062}$ & $0.92_{-0.39}^{+0.23}$ & $0.0506_{-0.0019}^{+0.0024}$ & $7.39_{-0.36}^{+0.36}$ & $0.39_{-0.27}^{+0.26}$ & $25.1741_{-0.0038}^{+0.0038}$ & $2855.6079_{-0.0025}^{+0.0025}$ & $0.33_{-0.22}^{+0.20}$ & $170_{-150}^{+10}$ \\
440150441 & 6648.01 &  & $1.215_{-0.034}^{+0.034}$ & $0.59_{-0.11}^{+0.11}$ & $0.53_{-0.34}^{+0.25}$ & $0.0326_{-0.0018}^{+0.0022}$ & $4.36_{-0.28}^{+0.29}$ & $0.47_{-0.32}^{+0.31}$ & $20.8616_{-0.0090}^{+0.0090}$ & $2879.9455_{-0.0054}^{+0.0054}$ & $0.03_{-0.03}^{+0.31}$ & $-30_{-150}^{+40}$ \\
441590110 & 5187.01 &  & $1.323_{-0.034}^{+0.034}$ & $0.468_{-0.060}^{+0.060}$ & $0.67_{-0.42}^{+0.29}$ & $0.0466_{-0.0023}^{+0.0027}$ & $6.76_{-0.39}^{+0.41}$ & $0.46_{-0.31}^{+0.31}$ & $17.85976_{-0.00017}^{+0.00017}$ & $2596.5067_{-0.0056}^{+0.0056}$ & $0.06_{-0.06}^{+0.32}$ & $-10_{-20}^{+180}$ \\
445805961 & 1710.01 & TOI-1710 b & $0.953_{-0.022}^{+0.022}$ & $1.16_{-0.12}^{+0.12}$ & $1.04_{-0.21}^{+0.10}$ & $0.04957_{-0.00073}^{+0.00087}$ & $5.16_{-0.14}^{+0.14}$ & $0.25_{-0.17}^{+0.20}$ & $24.283371_{-0.000030}^{+0.000030}$ & $3439.6657_{-0.0014}^{+0.0014}$ & $0.01_{-0.01}^{+0.22}$ & $-20_{-150}^{+10}$ \\
451606970 & 1214.01 &  & $0.855_{-0.021}^{+0.021}$ & $1.31_{-0.21}^{+0.21}$ & $1.38_{-0.92}^{+0.70}$ & $0.0224_{-0.0011}^{+0.0012}$ & $2.10_{-0.12}^{+0.11}$ & $0.51_{-0.35}^{+0.30}$ & $19.180781_{-0.000084}^{+0.000084}$ & $1634.5497_{-0.0038}^{+0.0038}$ & $0.00_{-0.00}^{+0.35}$ & $-20_{-160}^{+50}$ \\
451645081 & 783.01 &  & $0.644_{-0.016}^{+0.016}$ & $2.54_{-0.23}^{+0.23}$ & $2.7_{-2.5}^{+3.2}$ & $0.030_{-0.004}^{+0.011}$ & $2.45_{-0.59}^{+0.40}$ & $0.59_{-0.40}^{+0.36}$ & $8.112483_{-0.000060}^{+0.000060}$ & $2312.1213_{-0.0054}^{+0.0054}$ & $0.03_{-0.03}^{+0.41}$ & $-10_{-170}^{+60}$ \\
456306892 & 5581.01 &  & $0.775_{-0.017}^{+0.017}$ & $1.77_{-0.16}^{+0.16}$ & $1.14_{-0.31}^{+0.80}$ & $0.1167_{-0.0083}^{+0.0091}$ & $9.91_{-0.85}^{+0.69}$ & $0.82_{-0.13}^{+0.05}$ & $33.53626_{-0.00025}^{+0.00025}$ & $2390.9748_{-0.0020}^{+0.0020}$ & $0.02_{-0.02}^{+0.39}$ & $-140_{-30}^{+140}$ \\
456862677 & 4515.01 & TOI-4515 b & $0.880_{-0.024}^{+0.024}$ & $1.21_{-0.16}^{+0.16}$ & $2.7_{-0.5}^{+1.0}$ & $0.1281_{-0.0060}^{+0.0036}$ & $12.13_{-0.54}^{+0.58}$ & $0.75_{-0.11}^{+0.05}$ & $15.266425_{-0.000095}^{+0.000095}$ & $2451.62316_{-0.00056}^{+0.00056}$ & $0.36_{-0.24}^{+0.21}$ & $10_{-0}^{+160}$ \\
459969957 & 1274.01 &  & $0.783_{-0.019}^{+0.019}$ & $1.66_{-0.16}^{+0.16}$ & $1.56_{-0.12}^{+0.16}$ & $0.1060_{-0.0016}^{+0.0012}$ & $9.03_{-0.27}^{+0.23}$ & $0.392_{-0.092}^{+0.058}$ & $19.320337_{-0.000010}^{+0.000010}$ & $2736.34061_{-0.00032}^{+0.00032}$ & $0.01_{-0.01}^{+0.19}$ & $-20_{-160}^{+10}$ \\
459970307 & 1154.01 &  & $0.925_{-0.019}^{+0.019}$ & $1.26_{-0.12}^{+0.12}$ & $1.00_{-0.58}^{+0.35}$ & $0.0268_{-0.0011}^{+0.0014}$ & $2.72_{-0.13}^{+0.14}$ & $0.45_{-0.30}^{+0.30}$ & $21.745506_{-0.000096}^{+0.000096}$ & $3339.3277_{-0.0036}^{+0.0036}$ & $0.05_{-0.05}^{+0.28}$ & $-150_{-20}^{+140}$ \\
461635621 & 4460.01 &  & $0.689_{-0.015}^{+0.015}$ & $2.25_{-0.19}^{+0.19}$ & $0.25_{-0.23}^{+0.36}$ & $0.027_{-0.004}^{+0.012}$ & $2.42_{-0.70}^{+0.49}$ & $0.58_{-0.39}^{+0.38}$ & $28.6653_{-0.0011}^{+0.0011}$ & $3437.065_{-0.036}^{+0.036}$ & $0.50_{-0.50}^{+0.50}$ & $180_{-180}^{+180}$ \\

